Properties of the gradient squared of the discrete Gaussian free field

In this paper we study the properties of the centered (norm of the) gradient squared of the discrete Gaussian free field in $U_{\epsilon}=U/\epsilon\cap \mathbb{Z}^d$, $U\subset \mathbb{R}^d$ and $d\geq 2$. The covariance structure of the field is a function of the transfer current matrix and this relates the model to a class of systems (e.g. height-one field of the Abelian sandpile model or pattern fields in dimer models) that have a Gaussian limit due to the rapid decay of the transfer current. Indeed, we prove that the properly rescaled field converges to white noise in an appropriate local Besov-H\"older space. Moreover, under a different rescaling, we determine the $k$-point correlation function and cumulants on $U_{\epsilon}$ and in the continuum limit as $\epsilon\to 0$. This result is related to the analogue limit for the height-one field of the Abelian sandpile (\citet{durre}), with the same conformally covariant property in $d=2$.

==> Intro.tex <==
\section{Introduction}

The Gaussian free field (GFF) is one of the most prominent and tractable random interface models.\comment[id=ac]{GFF not a random interface, DGFF is. Distinguish between GFF and DGFF?}
The GFF appears as scaling limit of observables in many interacting particle systems, see e.g. \citet{Kenyon,Wilson2011XORIsingLA,jerison}. 
Moreover, the GFF acts as a building block for defining the Liouville measure in Liouville quantum gravity, \citet{beresticky}.\comment[id=ac]{ADD TO DO}


A (random) interface model is defined as a collection of (random) real heights $\Gamma=(\Gamma(x))_{x\in \Lambda}$, where \replaced[id=ac,comment={replaced $U$ with $\Lambda$ since graph needed to define an interface}]{$\Lambda$}{$U$} is a graph, measuring the vertical distance between the interface and the set $\Lambda$ in each point, \highlight[id=ac,comment={redundant}]{drawn from some probability measure}, see e.g. \citet{funaki}. In particular the probability measure for the GFF is a Gibbs measure with formal Hamiltonian given by \added[id=ac,comment={boundary cond?}]{In the present case, we will specialize to the case $\Lambda\subseteq \Z^d$. There we will set the DGFF measure to be the Gibbs measure with (formal) Hamiltonian given by
\[
    H(\Gamma) = \frac{1}{2d}\sum_{x,y: \|x-y\|=1} V\left(\Gamma(x)-\Gamma(y)\right) \ ,
\]
where $V(\varphi)=\varphi^2/2$.} \added[id=ac]{For general $V(\cdot)$ the above Hamiltonian defines a class of interfaces for which} There has been a lot of activity in studying properties such as decay of correlations or scaling limits \replaced[id=ac,comment={watch}]{for general potentials $V$}. In fact, the scaling limit will be the GFF if $V$ is even (\citet{NadafSpencer}), a convex (\citet{funaki}) or a \highlight[id=ac,comment={not true for all non-convex potentials, specify}]{general non-convex potential} $V$, see \citet{BiskupSpohn} and references therein. 

The gradient Gaussian free field $\nabla \Gamma$ is defined as the gradient of the field $\Gamma$, where $\Gamma$ has Gibbs distribution with quadratic potential \added[id=ac]{$V(\varphi)=\varphi^2/2$}. Its correlation structure \replaced[id=ac]{can be found}{was studied} e.g. in \citet{funaki}. This field on a discretized domain \highlight[id=ac,comment={can skip this}]{$D'=D\cap \mathbb{Z}^d$} is particularly interesting since its covariance structure can be written in terms of the transfer current matrix (see e.g. \citet{kassel-wu})
\[
\mathbb{E}\left[\nabla_i \Gamma(x) \nabla_j \Gamma(y)\right] = T(e,f) \ ,
\]
where $e=(x,x+e_i)$ and $f=(y,y+e_j)$ \added[id=ac]{are directed edges} and $\{e_i\}_i$ denotes the orthonormal basis of $\mathbb{R}^d$.
$T(e,f)$ describes a {\it current flow} between \deleted[id=ac]{directed edges} $e$ and $f$. The celebrated {\it transfer current theorem} of \citet{Burton} connects the spanning tree measure viewed as a point process on a set of undirected edges of a graph with the transfer current matrix by noticing that it is determinantal with kernel $T$. In Theorem 2 of \citet{kassel-wu}, the authors prove that for finite weighted graphs the rescaled correlations of the spanning tree model have a universal conformal covariant limit when $d=2$.

An interesting point mentioned in \citet{kassel-wu} is that the specific local statistics of models \added[id=ac]{which are closely related to the spanning tree measure}, e.g. spanning unicycle, Abelian sandpile \citet{durre} or dimer model \citet{Bouti} have a universal Gaussian limit. 

The specific local statistics or {\it pattern fields} are realizations of a random process in a subregion with the property that the local dependence translates into local dependence of the corresponding spanning tree. This is true for example for the field corresponding to minimal heights for the Abelian sandpile model, \citet{durre,durrethesis}. Correlations of those pattern fields can be expressed in terms of transfer current matrices which decay sufficiently fast and assure the central limit type of behaviour, \citet{Newman1980Jan}. 

In this paper we consider the recentered square of the gradient DGFF, formally denoted by $\Phi_{\eps}=\,:\!(\nabla \Gamma)^2\!:\,$, on a discretized domain $U_{\eps} = U/\eps \cap \mathbb{Z}^d$, $\eps>0$, $d\geq 2$. Let us remark that we do not consider $d=1$ here since the gradient of the DGFF will be just a sum of i.i.d. Gaussian variables.

Our first main result 
determines the $k$-point correlation function for the field $\Phi_{\eps}$ on the discretized domain and in the scaling limit as $\eps\to 0$.
\begin{theorem*}$1.$
For any $k \in \mathbb{N}$, $\eps>0$,
\begin{equation*}
    \E\left[\Phi_\eps\big(x_1\big) \cdots \Phi_{\eps}(x_k)\right] = \sum_{\pi }\prod_{B \in\pi}C_{|B|}\sum_{\sigma, \eta } \prod_{j\in B} \nabla_{\eta(j)}^{(1)}\nabla_{\eta(\sigma(j))}^{(2)}G_{U_\eps}\big(x^{(j)},x^{(\sigma(j))}\big) \,
\end{equation*}
where $G_{U_{\eps}}(\cdot,\cdot)$ is the Green's function on $U_{\eps}$.
Moreover, we have the convergence as $\eps\to  0$
\[    \lim_{\eps\to 0} \eps^{-dk}\E\left[\Phi_\eps\big(x_1\big) \cdots \Phi_{\eps}(x_k)\right] = \sum_{\pi}\prod_{B}C_{|B|}
    \sum_{\sigma, \eta} 
\prod_{j\in B} \partial_{\eta(j)}^{(1)}\partial_{\eta(\sigma(j))}^{(2)}G_U \big(x^{(j)}, x^{(\sigma(j))}\big).
\]
\end{theorem*}
As a corollary we also determine the corresponding cumulants on the discretized domain and in the scaling limit. In $d=2$ we show in Proposition \ref{thm:conformal} that the $k$-point correlation functions are conformally covariant.

The second main result is the scaling limit of the rescaled field towards white noise in some appropriate local Besov space, \citet{mourratarmstrong}. 

\begin{theorem*}$2.$
The gradient squared of the discrete Gaussian free field $\Phi_{\eps}$  converges to white noise as $\eps\to0$:
    \[
         \frac{\eps^{-d/2}}{\sqrt{\chi}} \Phi_{\eps} \overset{d}\longrightarrow W,
    \]
for some explicit constant \added[id=ac]{$\chi>0$}.
\end{theorem*}
The constant $\chi$, defined explicitly in~\eqref{eq:chi_def}, plays a special role since it is related to the sum over all covariances of the field $\Phi_{\eps}$ which turns out to be finite. Let us remark that this result is consistent with the result of \citet{Newman1980Jan}
where he proofs that translation invariant fields with finite covariance structure (susceptibility) satisfying the FKG inequality have a Gaussian limit. In our case we do not have translation invariance since we work on a domain.

The main idea for the proof of Theorem 1 is to decompose the $k$-point function in terms of complete Feynman diagrams, \citet{janson}. Then we can use the Gaussian nature of the field in order to write the product as products of covariances which can be expressed as transfer currents. To determine the scaling limit we will use expansions from \citet{funaki} and \citet{kassel-wu}. Let us stress that the 
proof differs from the one of \citet{durre} who uses the correspondence of the height one field and spanning tree explicitly to determine the $k$- point function and cumulants of the field. A notable observation is that his cumulants differ from ours by a minus sign hence do not represent the same field albeit belonging to the same universality class.

The proof of the second theorem is divided into two parts. In a first step we prove that the family of fields is tight in some appropriate local Besov space by using a tightness criterion of \citet{mf}. The second step consists of determining the finite dimensional distributions and identifying the limiting field. We rely on and generalize bounds on double gradients of the Green's function from \citet{lawlerlimic} and \citet{durre}.

The novelty of the paper lies in the fact that we constructed the gradient squared of the Gaussian free field on a discretized domain, determined its $k$-point correlation function and scaling limit. We identified the local Besov space where the field is living, which was not done in previous works, e.g. \citet{kassel-wu}.
This field lies in the same universality class as models which are connected to the spanning tree measure since it shares the covariance structure involving the transfer current matrix.


The structure of the paper is as follows. In Section \ref{sec:not} we fix notation, introduce the fields that we study and provide the definition of the local Besov spaces where convergence takes place. Section \ref{sec:main} is devoted to stating the main results. The subsequent Section \ref{sec:proofs} contains all proofs and finally in Section \ref{sec:dis} we discuss possible generalizations and pose open questions.

==> Intro2.tex <==
\section{Introduction}


The Gaussian free field (GFF) is one of the most prominent models for random surfaces. It appears as scaling limit of observables in many interacting particle systems, see for example \citet{Kenyon,Wilson2011XORIsingLA,jerison,Sheffield2007Nov}. It serves as a building block for defining the Liouville measure in Liouville quantum gravity (see \citet{Ding2021Sep} and references therein for a list of works on the topic). 

Its discrete counterpart, the discrete Gaussian free field (DGFF), is also very well-known among random interface models on graphs. Given a graph $\Lambda$, a (random) interface model is defined as a collection of (random) real heights $\Gamma=(\Gamma(x))_{x\in \Lambda}$, measuring the vertical distance between the interface and the set of points of $\Lambda$ (\citet{funaki,Velenik2006Jan}). The discrete Gaussian free field has attracted a lot of attention due to its links to random walks, cover times of graphs, and conformally invariant processes (see \citet{Glimm, Barlow,Sheffield2007Nov,Ding2012,Schramm2009Jan}, among others). In the present paper, we will consider the DGFF on the square lattice, that is, we will focus on $\Lambda\subseteq \Z^d$, in which case the probability measure of the DGFF is a Gibbs measure with formal Hamiltonian given by
\begin{equation}\label{eq:Hamiltonian}
    H(\Gamma) = \frac{1}{2d}\sum_{x,\,y: \|x-y\|=1} V\left(\Gamma(x)-\Gamma(y)\right) \ ,
\end{equation}
where $V(\varphi)=\varphi^2/2$. We will always work with $0$-boundary conditions, meaning that we will set $\Gamma(x)$ to be zero almost surely outside $\Lambda$. For general potentials $V(\cdot)$ the Hamiltonian~\eqref{eq:Hamiltonian} defines a broad class of gradient interfaces which have been widely studied in terms of decay of correlations and scaling limits~(\citet{NadafSpencer,BiskupSpohn,cotar2009strict}), among others.

The gradient Gaussian free field $\nabla \Gamma$ is defined as the gradient of the DGFF $\Gamma$ along edges of the square lattice. %where $\Gamma$ is a DGFF on $\Lambda \subset \Z^d$ with $0$-boundary conditions outside $\Lambda$.
This field is a centered Gaussian process whose correlation structure can be written in terms of $T(\cdot,\,\cdot)$, the transfer current (or transfer impedance) matrix (\citet{kassel-wu}). Namely, if we consider the gradient $\nabla_i \Gamma(\cdot)\coloneqq\Gamma(\cdot+e_i)-\Gamma(\cdot)$ in the $i$-th coordinate direction of $\R^d$, we have, for $x,\,y\in\Z^d,\,1\le i,\,j\le d $, that
\[
\begin{split}
    \mathbb{E}\left[\nabla_i \Gamma(x) \nabla_j \Gamma(y)\right] & = G_{\Lambda}(x,y) - G_{\Lambda}(x+e_i,y) -G_{\Lambda}(x,y+e_j) + G_{\Lambda}(x+e_i,y+e_j)  \\
    &= T(e,f)
\end{split}
\]
where  $e=(x,x+e_i)$ and $f=(y,y+e_j)$ are directed edges of the grid and $G_{\Lambda}(\cdot,\cdot)$ is the discrete harmonic Green's function on $\Lambda$ with $0$-boundary conditions outside $\Lambda$.
Here $T(e,f)$ describes a {current flow} between $e$ and $f$.

The main object we will study in our article is the following. Take $U$ to be a smooth, connected, bounded subset of $\R^d$. Consider the recentered squared norm of the gradient DGFF, formally denoted by $$\Phi_\eps(\cdot)=\,:\!\|\nabla \Gamma\|^2\!:\!(\cdot) =\sum_{i=1}^d : \left(\Gamma(\cdot+e_i)-\Gamma(\cdot)\right)^2 :$$
on the discretized domain $U_{\eps} = U/\eps \cap \mathbb{Z}^d$, $\eps>0$, $d\geq 2$, with $\Gamma$ a $0$-boundary DGFF on $U_\eps$. The colon $:(\cdot) :$ denotes the Wick centering of the random variables. In the rest of the paper we will simply call $\Phi_\eps$ {\em the gradient squared of the DGFF}. Let us remark that we do not consider $d=1$ here since in one dimension the gradient of the DGFF is a collection of i.i.d. Gaussian variables.


\subsection*{\texorpdfstring{$k$}{k}-point correlation functions}

Our first main result  determines the $k$-point correlation functions for the field $\Phi_{\eps}$ on the discretized domain $U_\eps$ and in the scaling limit as $\eps\to 0$. We defer the precise statement to Theorem~\ref{thm:cumulants} in Section \ref{sec:main}, which we will now expose in a more informal way. Let $\eps>0$ and $k \in \mathbb{N}$ and let the points $x^{(1)},\dots,x^{(k)}$ in $U \subset \R^d$, $d\geq 2$, be given. Define $x^{(j)}_\eps$ to be a discrete approximation of $x^{(j)}$ in $U_\eps$, for $j = 1,\dots,k$. Let $\Pi([k])$ be the set of partitions of $k$ objects and $S_\mathrm{cycl}^0(B) $ be the set of cyclic permutations of a set $B$ without fixed points. Finally let $\mathcal E$ be the set of coordinate vectors of $\R^d$. Then the $k$-point correlation function at fixed ``level'' $\eps$ is equal to
\begin{equation}\label{eq:cumulantsIntro}
    \E\left[\prod_{j=1}^k{\Phi_\eps\big(x^{(j)}_\eps\big)}\right] = \sum_{\pi\in\Pi([k])}\prod_{B\in\pi}2^{|B|-1}\sum_{\sigma\in S_\mathrm{cycl}^0(B)} \sum_{\eta:B\to\mathcal{E}}\prod_{j\in B} \nabla_{\eta(j)}^{(1)}\nabla_{\eta(\sigma(j))}^{(2)}G_{U_\eps}\big(x^{(j)}_\eps,x^{(\sigma(j))}_\eps\big).
\end{equation}
Moreover if $x^{(i)} \neq x^{(j)}$ for all $i \neq j$, the scaling limit of the above expression is
\begin{multline}\label{eq:moments_limitIntro}
    \lim_{\eps\to 0} \eps^{-dk}\E\left[\prod_{j=1}^k{\Phi_\eps\big(x^{(j)}_\eps\big)}\right] = \sum_{\pi\in\Pi([k])}\prod_{B\in\pi}2^{|B|-1}
    \sum_{\sigma\in S_\mathrm{cycl}^0(B)} \\
    \sum_{\eta:B\to\mathcal{E}}\prod_{j\in B} \partial_{\eta(j)}^{(1)}\partial_{\eta(\sigma(j))}^{(2)}G_U \big(x^{(j)}, x^{(\sigma(j))}\big) \,
\end{multline}
where $G_U(\cdot,\,\cdot)$ is the continuum Dirichlet harmonic Green's function on $U$. As a corollary (Corollary \ref{cor:cumulants}) we also determine the corresponding cumulants on $U_\eps$ and in the scaling limit.

Let us discuss some interesting observations in the sequel. The $k$-point correlation function of~\eqref{eq:moments_limitIntro} has similarities to the $k$-point correlation that arises in permanental processes, see \citet{Last, Eisen, manju} for relevant literature. In fact, in $d=1$ one can show that the gradient squared is {\em exactly} a permanental process with kernel given by the diagonal matrix whose non-zero entries are the double derivatives of $G_U$~\cite[Theorem 1]{mccullagh2006permanental}. In higher dimensions however we cannot identify a permanental process arising from the scaling limit, since the directions of derivations of the DGFF at each point are not independent. Nevertheless the 2-point correlation functions of $\Phi_\eps$ are positive (see Equation \eqref{eq:2point} in Section \ref{sec:proofs}), which is consistent with attractiveness of permanental processes \citep[Remark on p. 139]{Last}, and the overall structure resembles closely that of permanental processes marginals.

In $d=2$, the limiting cumulants $\kappa$ of our field are interestingly connected to the cumulants of the height-one field  $\big(h_{\eps}(x_{\eps}^{(i)}):\ x_\eps^{(i)}\in U_{\eps}\big)$ of the Abelian sandpile model~\citep[Theorem 2]{durre}. Theorem~\ref{thm:cumulants} will imply that for every set of $\ell\ge 2$ pairwise distinct points in $d=2$ one has
\begin{equation}\label{eq:equal_cumulants}
   -2\ \lim_{\eps\to 0} \eps^{-2 \ell}\kappa\left(\frac{C}{2}\Phi_\eps\big(x^{(1)}_\eps \big), \dots, \frac{C}{2}\Phi_\eps\big(x^{(\ell)}_\eps\big)\right) = \lim_{\eps\to 0} \eps^{-2 \ell}\kappa\left(h_\eps\big(x_{\eps}^{(1)} \big), \dots, h_\eps\big(x_{\eps}^{(\ell)}\big)\right)
\end{equation}
with 
\begin{equation}\label{eq:def_C}C=\frac{2}{\pi} -\frac{4}{\pi^2} =\pi \ \mathbb{E}\left(h_{0}(0)\right),\end{equation}
see \citet[Theorem 6]{durrethesis}.

We would also like to point out that the apparently intricate structure of Equations~\eqref{eq:cumulantsIntro}--\eqref{eq:moments_limitIntro} and of D\"urre's Theorem 2 can be unfolded as soon as one recognizes therein the structure of a Fock space. We will discuss this point in more detail in Subsection~\ref{subsec:fock}, where in particular in Corollary~\ref{cor:cum_in_height} we will derive a Fock space representation of the $k$-point function for the height-one field. We will pose further questions on this matter in the Discussion Section~\ref{sec:dis}.

Due to the similar nature of the cumulants in the height-one field of the sandpile and our field, we show in Proposition \ref{thm:conformal} that in $d=2$ the $k$-point correlation functions are conformally covariant (compare~\citet[Theorem 1]{durre},~\citet[Theorem 2]{kassel-wu}). This hints at Theorems 2 and 3 of \citet{kassel-wu}, in which the authors prove that for finite weighted graphs the rescaled correlations of the spanning tree model and minimal subconfigurations of the Abelian sandpile have a universal and conformally covariant limit. 


\subsection*{Scaling limit}

The second main result of our paper is the scaling limit of the field towards white noise in some appropriate local Besov-H\"older space. As we will show in Theorem~\ref{thm:goes_to_WN}, Section \ref{sec:main}, as $\eps\to0$ the gradient squared of the discrete Gaussian free field $\Phi_{\eps}$ converges as a random distribution to spatial white noise $W$:
\begin{equation}\label{eq:wn_intro}
         \frac{\eps^{-d/2}}{\sqrt{\chi}} \Phi_{\eps} \overset{d}\longrightarrow W \ ,
\end{equation}
for some explicit constant $0<\chi<\infty$. The result is sharp in the sense that we obtain convergence in the smallest H\"older space where white noise lives. The constant $\chi$, defined explicitly in~\eqref{eq:chi_def}, is the analogue of the susceptibility for the Ising model, in that it is a sum of all the covariances between the origin and any other lattice point.
We will prove that this constant is finite and the field $\Phi_\eps$ has a Gaussian limit. 
Note that \citet{Newman1980Jan} proves the same result
for translation-invariant fields with finite susceptibility satisfying the FKG inequality. In our case we do not have translation invariance since we work on a domain, so we are not able to apply directly this criterion. From a broader perspective there are several other results in the literature that obtain white noise in the limit due to an algebraic decay of the correlations, see for example~\citet{bauerschmidt2014scaling}.

Note that our field can be understood in a wider class of models having correlations which depend on the transfer current matrix $T(\cdot,\cdot)$. An interesting point mentioned in \citet{kassel-wu} is that pattern fields of determinantal processes closely connected to the spanning tree measure and $T(\cdot,\,\cdot)$ (for example the spanning unicycle, the Abelian sandpile model (\citet{durre}) and the dimer model (\citet{Bouti})) 
have a universal Gaussian limit when viewed as random distributions. Correlations of those pattern fields can be expressed in terms of transfer current matrices which decay sufficiently fast and assure the central limit-type behaviour which we also obtain. 



Let us comment finally on the differences between expressions \eqref{eq:moments_limitIntro} and~\eqref{eq:wn_intro}. The scaling factors are different, and this reflects two viewpoints one can have on $\Phi_\eps$: the one of \eqref{eq:moments_limitIntro} is that of correlation functionals in a Fock space, while in \eqref{eq:wn_intro} we are looking at it as a Gaussian distributional field (compare also Theorems 2 and 3 in~\citet{durre}). This is compatible, as there are examples of trivial correlation functionals which are non-zero as random distributions~(\citet{kang2013gaussian}).

The novelty of the paper lies in the fact that we construct the gradient squared of the Gaussian free field on a grid, determine its $k$-point correlation function and scaling limits. We determine tightness in optimal Besov-H\"older spaces (optimal in the sense that we cannot achieve a better regularity for the scaling limit to hold). Furthermore we show the ``dual'' behavior in the scaling limit of the gradient squared of the DGFF as a Fock space field and as a random distribution. As mentioned before we recognize a similarity to permanental processes, and it is worthwhile noticing that for general point processes there is a Fock space structure, see e.g. \citet[Section 18]{Last}. Since there is a close connection to the height-one field via correlation structures, we also unveil a Fock space structure in the Abelian sandpile model.

\subsection*{Proof ideas}

The main idea for the proof of results \eqref{eq:cumulantsIntro}--\eqref{eq:moments_limitIntro} is to decompose the $k$-point correlation function in terms of complete Feynman diagrams~(\citet{janson}). Then we can use the Gaussian nature of the field to expand the products of covariances as transfer currents. To determine the scaling limit we will use developments from \citet{funaki} and \citet{kassel-wu}. Let us stress that the proof of the scaling limit of cumulants differs from the one of \citet[Theorem 2]{durre} who instead uses the correspondence between the height-one field and the spanning tree explicitly to determine the limiting observables.

The proof of the scaling limit~\eqref{eq:wn_intro} is divided into two parts. In a first step (Proposition~\ref{thm:tightness}) we prove that the family of fields under consideration is tight in an appropriate local Besov-H\"older space by using a tightness criterion of \citet{mf}. The proof requires a precise control of the summability of $k$-point functions, which is provided by Theorem~\ref{thm:cumulants} and explicit estimates for double derivatives of the Green's function in a domain. Observe that, even if the proof relies on the knowledge of the joint moments of the family of fields, we only use asymptotic bounds derived from them. More specifically, we need to control the rate of growth of sums of moments at different points. The second step (Proposition~\ref{prop:convWN}) consists in determining the finite-dimensional distributions and identifying the limiting field. We will first show that the limiting distribution, when tested against test functions, has vanishing cumulants of order higher or equal to three, and secondly that the limiting covariance structure is the $L^2(U)$ inner product of the test functions. This will imply that the finite-dimensional distributions of converge to those corresponding to $d$-dimensional white noise. For this we rely on generalized bounds on double gradients of the Green's function from \citet{lawlerlimic} and \citet{durre}.


\paragraph{Structure of the paper} The structure of the paper is as follows. In Section \ref{sec:not} we fix notation, introduce the fields that we study and provide the definition of the local Besov-H\"older spaces where convergence takes place. Section \ref{sec:main} is devoted to stating the main results in a more precise manner. The subsequent Section \ref{sec:proofs} contains all proofs and finally in Section \ref{sec:dis} we discuss possible generalizations and pose open questions.

==> Old_files/tightness.tex <==
\section{Tightness criterion}

Following M-F paper, we will use their tightness criterion to prove the convergence of (some scaling of) our field.

Let $\Lambda_n \coloneqq \Z^d/2^n$, and let $R$ be such that
\begin{equation}\label{eq:support}
    \supp{f} \subset B_0(R) \quad , \quad \supp{g^{(i)}} \subset B_0(R) \ , \ i < 2^d \ .
\end{equation}
Let $K \subset U$ be compact and $k \in \N$. We say that the pair $(K, k)$ is \emph{adapted} if
\begin{equation}
    2^{-k}R < \dist{(K,U^c)} \ .
\end{equation}
We say that the set $\mathcal K$ is a \emph{spanning sequence} if it can be written as
\begin{equation}
    \mathcal K = \left\{(K_n,k_n), n \in \N\right\} \ ,
\end{equation}
where $(K_n)$ is an increasing sequence of compact subsets of $U$ such that $\bigcup_n K_n = U$, and for every $n$ the pair $(K_n, k_n)$ is adapted.

The tightness criterion now reads:

\begin{theorem}[Tightness criterion]\label{thm:criterion}
Let $f, (g^{(i)})_{1\leq i<2^d}$ in $\mathcal C^r_c$ with the support properties mentioned above, and fix $p\in[1,\infty), q\in[1,\infty]$ and $\alpha,\beta\in\R$ satisfying $\abs{\alpha}, \abs{\beta} < r, \alpha<\beta$. Let $(\Phi_m)_{m\in\N}$ be a family of random linear forms on $C_c^r(U)$, and let $\mathcal K$ be a spanning sequence. Assume that for every $(K, k) \in \mathcal K$ , there exists a constant $c = c(K,k) < \infty$ such that for every $m \in N$,
\begin{equation}\label{eq:crit_1}
    \sup_{x\in\Lambda_k\cap K}{\E\left[\abs{\big\langle \Phi_m,f\big(2^k(\cdot-x)\big)\big\rangle}^p\right]^{1/p}} \leq C
\end{equation}
and
\begin{equation}\label{eq:crit_2}
    \sup_{x\in\Lambda_n\cap K}{2^{dn}\E\left[\abs{\big\langle \Phi_m,g^{(i)}\big(2^n(\cdot-x)\big)\big\rangle}^p\right]^{1/p}} \leq C \, 2^{-n\beta} \quad , \quad i<2^d,\, n\geq k \ .
\end{equation}
Then the family $(\Phi_m)$ is tight in $\mathcal{B}^{\alpha,\mathrm{loc}}_{p,q}(U)$. If moreover $\alpha < \beta - \frac d p$, then the family is also tight in $\mathcal C^\alpha_\mathrm{loc}(U)$.
\end{theorem}


\section{Tightness of the field}

\textcolor{red}{REMEMBER: in all this proof, when using the bound $\nabla\nabla G < c_D \abs{x-y}^{-2}$, that constant DEPENDS on the compact set $D$ and all that. It breaks on the boundary otherwise.}

We now proceed to apply the criterion \ref{thm:criterion} to our field. We will use an arbitrary scaling $\eps^{\gamma}, \gamma \in\R$, so that we can see which scalings make the fields tight and in which spaces. To simplify notation, we redefine $\Phi_\eps$ as
\[
    \Phi_\eps(x) \coloneqq \eps^\gamma \sum_{i=1}^2{:{\mathrm{d}\Gamma}^2_i(x):} \quad , \quad x \in V_\eps \ .
\]
The family of random linear forms $(\Phi_m)_{m\in\N}$ is to be identified with the fields $(\Phi_\eps)_{\eps>0}$. Now let us expand the expressions \eqref{eq:crit_1} and \eqref{eq:crit_2}. For simplicity of notation, let us define $f_{k,x}(\cdot) \coloneqq f\big(2^k(\cdot-x)\big)$, and analogously for $g^{(i)}$.

As for \eqref{eq:crit_1}, we have
\begin{equation}\label{eq:crit_1_1}
    \E\left[\abs{\big\langle \Phi_\eps,f_{k,x}\big\rangle}^p\right] = \eps^{\gamma p} \int{\E\left[\Phi_\eps\left(\floor{x_1/\eps}\right)\dots\Phi_\eps\left(\floor{x_p/\eps}\right)\right] f_{k,x}(x_1)\dots f_{k,x}(x_p)\, \d x_1\dots\d x_p} \ .
\end{equation}
However, we will seek for a more convenient expression to work with. We first note that $\Phi_\eps$ can be also expressed in a piece-wise continuous fashion as
\[
    \Phi_\eps(x) = \eps^{\gamma} \sum_{y\in U_\eps} \1_{S_1(y)}(x) \sum_{i=1}^2{:\d\Gamma^2_i(y):}
\]
\marginnote{See if this definition of S with vertex in y instead of centre conflicts with the proof below}where $S_a(y)$ is the square $\big[y^{(1)},y^{(1)}+a\big]\times\big[y^{(2)},y^{(2)}+a\big]$, with $y^{(1)}$ and $y^{(2)}$ the first and second components of $y$, respectively. This way, expression \eqref{eq:crit_1_1} now reads
\vspace{2cm}
%%%
\begin{equation}
    \int\int dx dy \varphi(x)\varphi(y)\E[\Phi_\eps(\floor{x/\eps})\Phi_\eps(\floor{y/\eps})]=\sum_{x_0,y_0\in U_\eps}\E[\Phi_\eps(x_0)\Phi_\eps(y_0)]\int_{x\in U:\floor{x/\eps}=x_0}\int_{y\in U:\floor{y/\eps}=y_0}\varphi(x)\varphi(y)dx dy
\end{equation}
%%%
\vspace{2cm}
%%%%%

\marginnote{Check if $S_\eps(\eps y_j)$ is correct.}
\[
    \E\left[\abs{\big\langle \Phi_\eps,f_{k,x}\big\rangle}^p\right] = \eps^{\gamma p} \sum_{y_1,\dots,y_p\in U_\eps} {\E\left[\sigma_{y_1}\dots\sigma_{y_p}\right]}\prod_{j=1}^p{\int_{S_\eps(\eps y_j)}{f_{k,x}(z) \,\d z}} \ ,
\]
where $\sigma_y \coloneqq \sum_{i=1}^2{:\d\Gamma^2_i(y):\,}$. Expression \eqref{eq:crit_1} now takes the form
\begin{equation}\label{eq:first}
    \eps^{\gamma} \sup_{x\in\Lambda_k \cap K}{\left[\sum_{y_1,\dots,y_p\in U_\eps} {\E\left[\sigma_{y_1}\dots\sigma_{y_p}\right]}\prod_{j=1}^p{\int_{S_\eps(\eps y_j)}{f_{k,x}(z) \,\d z}}\right]^{1/p}} \ .
\end{equation}
Analogously, expression \eqref{eq:crit_2} reads
\begin{equation}\label{eq:second}
    \eps^{\gamma} \, 2^{2n}\sup_{x\in\Lambda_n \cap K}{\left[\sum_{y_1,\dots,y_p\in U_\eps} {\E\left[\sigma_{y_1}\dots\sigma_{y_p}\right]}\prod_{j=1}^p{\int_{S_\eps(\eps y_j)}{g_{n,x}^{(i)}(z) \,\d z}}\right]^{1/p}} \ .
\end{equation}

We now proceed to the proof. First let us start by setting the spanning sequence. We choose $\mathcal K = (K_n,n)_{n\in\N}$, with
\[
    K_n = \big\{x\in\R^2 \mid \dist{(x,U^c)}\geq(2+\delta)R2^{-n}\big\} \ ,
\]
for some $\delta > 0$ and $R$ such that \eqref{eq:support} holds.

\marginnote{\textcolor{red}{If this is going to the paper, paraphrase these things because some of them are very similar to M-F's}}Let us first consider \eqref{eq:second}. Given that $\supp{g^{(i)}\big(2^n(\cdot-x)\big)} \subset B_x(R2^{-n})$ we can restrict the sum over $y_j$ to the set
\[
    \Omega_{n,x} = \left\{y\in U_\eps \mid \d(y,x)<2^{-n}R+\eps/\sqrt{2}\right\} \ .
\]
Now we bound \eqref{eq:second} separately for the cases $2^n \geq R\eps^{-1}$ and $2^n < R\eps^{-1}$.

If $2^n \geq R\eps^{-1}$, we have
\begin{multline*}
    \sum_{y_1,\dots,y_p\in U_\eps} {\E\left[\sigma_{y_1}\dots\sigma_{y_p}\right]}\prod_{j=1}^p{\int_{S_\eps(\eps y_j)}{g_{n,x}^{(i)}(z) \,\d z}} \leq \\
    \leq \sum_{y_1,\dots,y_p\in \Omega_{n,x}} {\E\left[\sigma_{y_1}\dots\sigma_{y_p}\right]}\prod_{j=1}^p{\int_{S_\eps(\eps y_j)}{g_{n,x}^{(i)}(z) \,\d z}} \ .
\end{multline*}
The sum over $\Omega_{n,x}$ can be bounded by a sum over a finite amount of points independent of $n$, and using the fact that
\[
    \int_{S_\eps(\eps y_j)}{g_{n,x}^{(i)}(z) \,\d z} \leq 2^{-2n} \ ,
\]
we obtain
\[
    \sum_{y_1,\dots,y_p\in \Omega_{n,x}} {\E\left[\sigma_{y_1}\dots\sigma_{y_p}\right]}\prod_{j=1}^p{\int_{S_\eps(\eps y_j)}{g_{n,x}^{(i)}(z) \,\d z}} \lesssim 2^{-2pn} \ ,
\]
which gives the bound
\[
    \eps^{\gamma} \, 2^{2n}\sup_{x\in\Lambda_n \cap K}{\left[\sum_{y_1,\dots,y_p\in U_\eps} {\E\left[\sigma_{y_1}\dots\sigma_{y_p}\right]}\prod_{j=1}^p{\int_{S_\eps(\eps y_j)}{g_{n,x}^{(i)}(z) \,\d z}}\right]^{1/p}} \lesssim \eps^{\gamma} \ .
\]
If $\gamma\leq0$ then we can bound the above expression as $\lesssim 2^{-\gamma n}$, whereas if $\gamma>0$ the expression can be bounded by any power of $2^n$ since $\eps$ is never greater than 1. \textcolor{red}{Is this last part for $\gamma>0$ true? It makes sense that for big $\gamma$ the field goes to 0 and there should be convergence in nicer spaces (probably of any desired regularity, like $\mathcal C^\infty$)}

On the other hand, if $2^n < R\eps^{-1}$, we have
\[
    \int_{S_\eps(\eps y_j)}{g_{n,x}^{(i)}(z)\d z} \leq \eps^2 \ .
\]
We also note that
\[
    \Omega_{n,x} \subset S_{\eps,x} \coloneqq \left[x - 2R2^{-n},x + 2R2^{-n}\right]^2 \cap \eps\Z^2 \ .
\]
Using this and calling $N\coloneqq\lfloor2R2^{-n}\eps^{-1}\rfloor$, we obtain
\[
    \sum_{y_1,\dots,y_p\in \Omega_{n,x}} {\E\left[\sigma_{y_1}\dots\sigma_{y_p}\right]} \leq \sum_{y_1,\dots,y_p\in \llbracket-N,N\rrbracket^2} {\E\left[\sigma_{y_1}\dots\sigma_{y_p}\right]} \ ,
\]
where the notation $\llbracket-N,N\rrbracket$ indicates the set $\{n\in\Z : -N\leq n\leq N\}$.

\textcolor{red}{IMPORTANT: Here (or above) I should mention the property of the bound of the double difference of the Green function. Also, keep in mind I know it works for $p=2$, but still not sure how to prove it for any $p$.}
From the cumulants expression for the field \eqref{eq:cumulants} we know that, for any $y_1,y_2$ in $U_\eps$,\marginnote{\textcolor{red}{Mention here that it also applies when some $y_i=y_j$}}
\[
    \E\big[\sigma_{y_1}\sigma_{y_2}\big] = 2 \sum_{j,k=1,2} \left(\nabla_j^{(1)}\nabla_k^{(2)}G_{U_\eps}(y_1,y_2)\right)^2 \ .
\]
Also, from \eqref{eq:two_duerre} there exists a constant $c_K>0$ possibly dependent of the compact set $K$ but independent of $y_1, y_2$ such that
\[
    \abs{\nabla_i^{(1)}\nabla_j^{(2)} G_{U_\eps}(y_1,y_2)} \leq c_K \cdot
    \begin{dcases}
        \abs{y_1-y_2}^{-2} \ &\text{if} \ y_1\neq y_2 \ ,\\
        1 \ &\text{if} \ y_1 = y_2 \ .
    \end{dcases}
\]
Hence \textcolor{red}{(explain this ``hence'')}
\[
    \sum_{y_1,y_2\in U_\eps} {\E\left[\sigma_{y_1}\sigma_{y_2}\right]} \lesssim \abs{U_\eps} \ .
\]
For an arbitrary $p$, $\E[\sigma_{y_1}\dots\sigma_{y_p}]$ is a sum of double differences of the discrete Green function to the power $p$. \textcolor{red}{And supposing this reasoning can be applied for any $p$ (I'm not sure though)}, we have
\begin{equation}\label{eq:dubious}
    \sum_{y_1,\dots,y_p\in U_\eps} {\E\left[\sigma_{y_1}\dots\sigma_{y_p}\right]} \lesssim \abs{U_\eps}^{p/2} \ .
\end{equation}
This implies that
\[
    \sum_{y_1,\dots,y_p\in \llbracket-N,N\rrbracket^2} {\E\left[\sigma_{y_1}\dots\sigma_{y_p}\right]} \lesssim N^p \lesssim 2^{-np}\eps^{-p} \ .
\]
Putting everything together,
\[
    \eps^{\gamma} \, 2^{2n}\sup_{x\in\Lambda_n \cap K}{\left[\sum_{y_1,\dots,y_p\in U_\eps} {\E\left[\sigma_{y_1}\dots\sigma_{y_p}\right]}\prod_{j=1}^p{\int_{S_\eps(\eps y_j)}{g_{n,x}^{(i)}(z) \,\d z}}\right]^{1/p}} \lesssim 2^n \eps^{\gamma+1}
\]
If $\gamma \geq -1$ then we can bound the above expression as $\lesssim 2^n 2^{(\gamma+1)n} = 2^{(\gamma+2)n}$. Otherwise, we cannot bound it uniformly in $\eps$, as the bound depends increasingly on $\eps$ as it approaches 0.

Now we need to obtain similar bounds for \eqref{eq:crit_1}, which applied to our case takes the expression given in \eqref{eq:first}. For the case $2^n \geq R\eps^{-1}$ we have
\[
    \eps^{\gamma} \sup_{x\in\Lambda_k \cap K}{\left[\sum_{y_1,\dots,y_p\in U_\eps} {\E\left[\sigma_{y_1}\dots\sigma_{y_p}\right]}\prod_{j=1}^p{\int_{S_\eps(\eps y_j)}{f_{k,x}(z) \,\d z}}\right]^{1/p}} \lesssim \eps^\gamma 2^{-2k} \ ,
\]
which is bounded by some $c = c(K,k)$ as required, independently of $\gamma$ (remember $\eps \leq 1$). If $2^n < R\eps^{-1}$,
\[
    \eps^{\gamma} \sup_{x\in\Lambda_k \cap K}{\left[\sum_{y_1,\dots,y_p\in U_\eps} {\E\left[\sigma_{y_1}\dots\sigma_{y_p}\right]}\prod_{j=1}^p{\int_{S_\eps(\eps y_j)}{f_{k,x}(z) \,\d z}}\right]^{1/p}} \lesssim \eps^{(\gamma+1)} 2^{-k} \ .
\]
As before, only if $\gamma \geq -1$ we have the required bound.

\marginnote{\textcolor{red}{Actually MF don't say this. They say that is is tight in $\mathcal B_{p,q}^{\alpha,\mathrm{loc}}$ for any $q\in[1,\infty]$, $\alpha < -1$, and any $p\in[1,\infty]$. But looking at the thm., can't we also conclude the statement for $\mathcal C^\alpha_\mathrm{loc}(U)$?}}Theorem \ref{thm:criterion} now implies that, with scaling $\eps^{-1}$ the family $(\Phi_\eps)$ is tight in $\mathcal C^\alpha_\mathrm{loc}(U)$ every $\alpha < -1$, but with scaling $\eps^{-2}$ we cannot apply the criterion to show tightness is any space.

\begin{remark}[\textcolor{red}{IMPORTANT!!}]
    I'm still not sure about expression \eqref{eq:dubious}. I am however sure that it works for $p=2$. So, let's in principle assume that we only know it for $p=2$ and not for larger $p$'s. In that case Theorem \ref{thm:criterion} tells us that we have tightness in $\mathcal B_{2,q}^{\alpha,\mathrm{loc}}$ for any $q\in[1,\infty]$ and $\alpha < -1$, and also in $\mathcal C^\alpha_\mathrm{loc}(U)$ every $\alpha < -2$.
\end{remark}

==> Old_files/variance.tex <==
\section{Variance}

We are interested in computing the limit for $\eps\to0$ of
\[
    \V\big[\left\langle\Phi_\eps,f\right\rangle\big] = \E\big[\left(\left\langle\Phi_\eps,f\right\rangle\right)^2\big] \ ,
\]
for $f \in \mathcal C_C^\infty(U)$. Since the domain of $\Phi_\eps$ is included in $\Z^2$, we have
\begin{equation}\label{eq:variance}
    \V\big[\left\langle\Phi_\eps,f\right\rangle\big] = \int_{U\times U} f(x) f(y)\, \E\left[\Phi_\eps\left(\floor{x/\eps}\right)\Phi_\eps\left(\floor{y/\eps}\right)\right] \d x\,\d y \ .
\end{equation}
We start by dividing the integral into two regions: $\norm{x-y} < \eps$ and $\norm{x-y} \geq \eps$. As for the first one, in this case $\floor{x/\eps} = \floor{y/\eps}$, so
\begin{equation}\label{eq:less_eps}
    \int\displaylimits_{\norm{x-y}<\eps} f(x) f(y) \, \E\left[\Phi_\eps\left(\floor{x/\eps}\right)\Phi_\eps\left(\floor{y/\eps}\right)\right] \d x\,\d y = \int\displaylimits_{\norm{x-y}<\eps} f(x) f(y) \V\left[\Phi_\eps\left(\floor{x/\eps}\right)\right] \d x\,\d y \ .
\end{equation}
From the expression of the cumulants \eqref{eq:cumulants} we know that the 2-point function for points $x,y$ is equal to\marginnote{\textcolor{red}{Check where to say that the 2-point function for the SAME point has the same form}}
\[
    2 \sum_{i,j=1,2}\big(\nabla_i^{(1)}\nabla_j^{(2)} G_{U_\eps}(x,y)\big)^2 \ .
\]
Since the variance $\V\left[\Phi_\eps\left(\floor{x/\eps}\right)\right]$ is the 2-point function evaluated at the same point $\floor{x/\eps}$, the integral \eqref{eq:less_eps} is equal to
\begin{multline*}
    2 \sum_{i,j=1,2} \, \int\displaylimits_{\norm{x-y}<\eps} f(x) f(y) \big(\nabla_i^{(1)}\nabla_j^{(2)} G_{U_\eps}\left(\floor{x/\eps},\floor{x/\eps}\right)\big)^2 \d x\,\d y =\\
    = 2 \sum_{i,j=1,2} \, \int_U f(x) \big(\nabla_i^{(1)}\nabla_j^{(2)} G_{U_\eps}\left(\floor{x/\eps},\floor{x/\eps}\right)\big)^2\, \d x\int_{B_\eps(x)\cap U} f(y) \,\d y
\end{multline*}
Then, under the scaling $\eps^{-1}$ for the field $\Phi_\eps$, if we take the limit of this expression we have
\begin{multline}\label{eq:limit_variance}
    \lim_{\eps\to0} \, 2 \sum_{i,j=1,2} \, \int_U f(x) \big(\nabla_i^{(1)}\nabla_j^{(2)} G_{U_\eps}\left(\floor{x/\eps},\floor{x/\eps}\right)\big)^2\, \d x\int_{B_\eps(x)\cap U} \eps^{-2} \, f(y) \,\d y = \\
    = 2\pi \sum_{i,j=1,2} \, \int_U f(x)^2 \lim_{\eps\to0} \big(\nabla_i^{(1)}\nabla_j^{(2)} G_{U_\eps}\left(\floor{x/\eps},\floor{x/\eps}\right)\big)^2\, \d x \ ,
\end{multline}
where we used the dominated convergence theorem (justified by~\eqref{eq:two_duerre} and the Cauchy--Schwarz inequality) to insert the limit inside the integral in $x$ and the Lebesgue differentiation theorem to replace the integral in $y$ by $f(x)$. From equation \eqref{eq:one_duerre} of Lemma \ref{lemma:bound_2_points_durre} we infer that, for $x\in U$
\begin{equation}\label{eq:green_diff}
    \abs{\nabla_i^{(1)}\nabla_j^{(2)} G_{U_\eps}\left(\floor{x/\eps},\floor{x/\eps}\right) - \nabla_i^{(1)}\nabla_j^{(2)} G_0\left(\floor{x/\eps},\floor{x/\eps}\right)} \leq c_x \, \eps^2 \ ,
\end{equation}
being $c_x$ a constant depending on the point $x$. With this result in mind, let us now express the limit of the 2-point function in terms of $G_0$. We can expand the double difference of $G_0$ as follows. For all $x\in\Z^2$,
\[
    \nabla_i^{(1)}\nabla_j^{(2)} G_0(x,x) = G_0(x+e_i,x+e_j) - G_0(x+e_i,x) - G_0(x,x+e_j) + G_0(x,x) \ .
\]
Let us remind ourselves that the classical Green's function $G_0$ can be expressed in terms of the so-called \emph{potential kernel} $a(\cdot)$ \citep[Section 12]{spitzer} as
\[
    G_0(x,y) = -\frac14 a(x-y) \ , \ x,y\in\Z^2 \ .
\]
Evaluating at $y=x$, and using the well-known values for the potential kernel (see \citet[Section 15]{spitzer}), we have
\[
    \nabla_i^{(1)}\nabla_j^{(2)} G_0(x,x) = 
    \begin{dcases}
    \hfil \frac12 \ &\text{if} \ i=j \ ,\\
    \frac12 - \frac1\pi \ &\text{if} \ i\neq j \ ,
    \end{dcases}
\]
for all $x\in\Z^2$. Using \eqref{eq:green_diff}, for all $x \in U$ we have
\[
    \lim_{\eps\to0} \nabla_i^{(1)}\nabla_j^{(2)} G_{U_\eps}\left(\floor{x/\eps},\floor{x/\eps}\right) = 
    \begin{dcases}
    \hfil \frac12 \ &\text{if} \ i=j \ ,\\
    \frac12 - \frac1\pi \ &\text{if} \ i\neq j \ .
    \end{dcases}
\]
Finally, \eqref{eq:limit_variance} reads
\begin{equation}\label{eq:conv_less_eps}
    \left[2\pi - 4 \left(1 - \frac1\pi\right)\right] \int_U f(x)^2 \, \d x = \left[2\pi - 4 \left(1 - \frac1\pi\right)\right] \norm{f}_{L^2} \ .
\end{equation}

Let us now analyse the region where $\norm{x-y}\geq\eps$. From Lemma \ref{lemma:bound_2_points_durre}, if $D\subset U$ is a compact set, then $\forall\, x,y \in D_\eps$ we have the bound
\[
   \abs{\nabla_{i,x}\nabla_{j,x'}G(x,x')} < c_D \abs{x-y}^{-2}
\]
uniformly in $x$ and $y$, with $c_D$ a constant depending on $D$. Hence, the expectation inside \eqref{eq:variance} for the region $\norm{x-y}\geq\eps$ is a sum of four terms, each of which can be bounded (up to a global constant) by
\[
    \int\displaylimits_{\norm{x-y}\geq\eps} f(x) f(y) \,\eps^4 \,\abs{x-y}^{-4} \d x\, \d y \ .
\]
Although this integral does not have, in general, a simple form solution as in \eqref{eq:conv_less_eps}, under the previous scaling $\eps^{-1}$ a simple change of variables shows that it is finite.

We see then that, for any scaling $\eps^\gamma$ with $\gamma\geq-1$, the variance of $\langle\Phi_\eps,f\rangle$ converges as $\eps\to0$, whereas it diverges for any $\gamma<-1$.

==> Old_files/variance2.tex <==
\section{Variance}

\paragraph{Bounded eccentricity sets} For this Section we need to show a preliminary Lemma. Define the set $\mathcal I$ made up by the grid points of $ [-1,1]^2\cap\Z^2$; that is,
\[
    \mathcal I = \left\{(0,0)^T,\,(1,0)^T,\,(1,1)^T,\,(0,1)^T,\,(-1,1)^T,\,(-1,0)^T,\,(-1,-1)^T,\,(0,-1)^T,\,(1,-1)^T\right\} \ .
\]
For $x\in U$ and $\iota \in\mathcal I$, call $$A_{\eps,\iota,\,x} \coloneqq \left\{y\in B_\eps(x):\floor{x/\eps}-\floor{y/\eps}=\iota\right\}$$
(see Figure~\ref{fig:A} for an example of such sets).
\begin{figure}[ht!]
    \centering
    \includegraphics[scale=.2]{TryAlan.png}
    \caption{An example of $A_{\eps,\iota,x}$ for $\iota=(-1,\,0)^T$}
    \label{fig:A}
\end{figure}
We are going to show that the sets $\{A_{\eps,\iota,\,x}:\,\eps\in[0,\,dist(x,\partial U)]\}$ are of size comparable to that of balls and as such they allow us to use the Lebesgue differentiation theorem. 

Let us be more specific. A collection of Lebesgue-measurable sets $\{A_\alpha\}$ has bounded eccentricity at $x$ if there exists a constant $c > 0 $ such that for
each $A_{\alpha}$ there is a ball $B$ with
$x\in B$ such that
$$
A_{\alpha}\subset B,\quad meas(A_{\alpha})\ge c\, meas(B)
$$
(see \citet[p. 108]{steinshakarchi}). We can prove
\begin{lemma}\label{lem:be}
For $x\in U,\,\iota \in\mathcal I$ fixed, the sets $\{A_{\eps,\iota,\,x}:\epsilon\in[0,\,dist(x,\,\partial U)\}$ have bounded eccentricity at $x$.
\end{lemma}
\begin{proof}
TO DISCUSS
\end{proof}
Lemma~\ref{lem:be} implies immediately~\citep[Corollary 1.7]{steinshakarchi} that one can apply the Lebesgue differentiation theorem on $A_{\eps,\iota,\,x}$, that is,
\begin{corollary}\label{cor:LDT}
If $f(\cdot)$ is a locally integrable function on $\R^d$ then
\begin{equation}
   \lim_{\eps\to 0}\frac{1}{meas(A_{\eps,\iota,\,x})}\int_{A_{\eps,\iota,\,x}}f(y)\d y=f(x).
\end{equation}
\end{corollary}
%%%%%%%%%%%%%%% Paragraph
\paragraph{Computation of the limit variance} We are interested in computing the limit for $\eps\to0$ of
\[
    \V\big[\left\langle\Phi_\eps,f\right\rangle\big] = \E\left[\left(\left\langle\Phi_\eps,f\right\rangle\right)^2\right] \ ,
\]
for $f \in \mathcal C_C^\infty(U)$. Since the domain of $\Phi_\eps$ is included in $\Z^2$, we have
\begin{equation}\label{eq:variance}
    \V\big[\left\langle\Phi_\eps,f\right\rangle\big] = \int_{U\times U} f(x) f(y)\, \E\left[\Phi_\eps\left(\floor{x/\eps}\right)\Phi_\eps\left(\floor{y/\eps}\right)\right] \d x\,\d y \ .
\end{equation}
We divide the integral into two regions: $\norm{x-y} < \eps$ and $\norm{x-y} \geq \eps$. We start by analysing the first one. From the expression of the cumulants \eqref{eq:cumulants} we know that the 2-point function for points $x,y$ is equal to
\[
    2 \sum_{i,j=1,2}\big(\nabla_i^{(1)}\nabla_j^{(2)} G_{U_\eps}(x,y)\big)^2 \ .
\]
Thus,
\begin{multline*}
    2 \sum_{i,j=1,2} \, \int\displaylimits_{\norm{x-y}<\eps} f(x) f(y) \big(\nabla_i^{(1)}\nabla_j^{(2)} G_{U_\eps}\left(\floor{x/\eps},\floor{y/\eps}\right)\big)^2 \d x\,\d y =\\
    = 2 \sum_{i,j=1,2} \, \int_U f(x) \,\d x \int_{B_\eps(x)\cap U} f(y) \,\d y \, \big(\nabla_i^{(1)}\nabla_j^{(2)} G_{U_\eps}\left(\floor{x/\eps},\floor{y/\eps}\right)\big)^2
\end{multline*}
Then, under the scaling $\eps^{-1}$ for the field $\Phi_\eps$, if we take the limit of this expression we have
\begin{multline}\label{eq:limit_variance}
    \lim_{\eps\to0} \, 2 \, \eps^{-2} \sum_{i,j=1,2} \, \int_U f(x) \,\d x \int_{B_\eps(x)\cap U} f(y) \,\d y \, \left(\nabla_i^{(1)}\nabla_j^{(2)} G_{U_\eps}\left(\floor{x/\eps},\floor{y/\eps}\right)\right)^2 = \\
    = 2 \sum_{i,j=1,2} \, \int_U f(x) \,\d x \,\lim_{\eps\to0} \, \int_{B_\eps(x)\cap U} \eps^{-2} \,f(y) \,\d y \, \left(\nabla_i^{(1)}\nabla_j^{(2)} G_{U_\eps}\left(\floor{x/\eps},\floor{y/\eps}\right)\right)^2 \\
    = 2 \sum_{i,j=1,2} \, \int_U f(x) \,\d x \sum_{\iota\in\mathcal I} \lim_{\eps\to0}\, \int_{A_{\eps,\iota}\cap U} \eps^{-2} \,f(y) \,\d y \, \left(\nabla_i^{(1)}\nabla_j^{(2)} G_{U_\eps}\left(\floor{x/\eps}, \floor{x/\eps}+\iota\right)\right)^2 \\
    = 2 \sum_{i,j=1,2} \, \int_U f(x) \,\d x \sum_{\iota\in\mathcal I} \lim_{\eps\to0}\, \left(\nabla_i^{(1)}\nabla_j^{(2)} G_{U_\eps}\left(\floor{x/\eps}, \floor{x/\eps}+\iota\right)\right)^2 \int_{A_{\eps,\iota} \cap U} \eps^{-2} \,f(y) \,\d y \ ,
\end{multline}
\marginpar{\textcolor{red}{I can't get $f(x)$ out of the integral of $f(y)$ using LDT.}}






where we used the dominated convergence theorem (justified by~\eqref{eq:two_duerre} and the Cauchy--Schwarz inequality) to insert the limit inside the integral in $x$ and Corollary~\ref{cor:LDT} to replace the integral in $y$ by $f(x)$. From equation \eqref{eq:one_duerre} of Lemma \ref{lemma:bound_2_points_durre} we infer that, for $x,y\in U$
\begin{equation}\label{eq:green_diff}
    \abs{\nabla_i^{(1)}\nabla_j^{(2)} G_{U_\eps}\left(\floor{x/\eps},\floor{y/\eps}\right) - \nabla_i^{(1)}\nabla_j^{(2)} G_0\left(\floor{x/\eps},\floor{y/\eps}\right)} \leq c_{x,y} \, \eps^2 \ ,
\end{equation}
being $c_{x,y}$ a constant depending on the points $x$ and $y$. With this result in mind, let us now express the limit of the 2-point function in terms of $G_0$. We can expand the double difference of $G_0$ as follows. For all $x,y\in\Z^2$,
\begin{equation}\label{eq:green_double_diff}
    \nabla_i^{(1)}\nabla_j^{(2)} G_0(x,y) = G_0(x+e_i,y+e_j) - G_0(x+e_i,y) - G_0(x,y+e_j) + G_0(x,y) \ .
\end{equation}
Let us remind ourselves that the classical Green's function $G_0$ can be expressed in terms of the so-called \emph{potential kernel} $a(\cdot)$ \citep[Section 12]{spitzer} as
\[
    G_0(x,y) = -\frac14 a(x-y) \ , \ x,y\in\Z^2 \ .
\]
Since $\norm{x-y} < \eps$, the possible values of $\floor{x/\eps} - \floor{y/\eps}$ are the points of $\mathcal I$. By the symmetry of the potential kernel, we only need to compute the cases where $\floor{x/\eps} - \floor{y/\eps}$ equals $(0,0)$, $(1,0)$ and $(1,1)$ (considering their respective multiplicity).

The case for $\floor{x/\eps} - \floor{y/\eps} = (0,0)$ implies computing \eqref{eq:green_double_diff} at $y=x$. Using the well-known values for the potential kernel (see \citet[Section 15]{spitzer}), we have
\[
    \nabla_i^{(1)}\nabla_j^{(2)} G_0(x,x) = 
    \begin{dcases}
    \hfil \frac12 \ &\text{if} \ i=j \ ,\\
    \frac12 - \frac1\pi \ &\text{if} \ i\neq j \ ,
    \end{dcases}
\]
for all $x\in\Z^2$. Using \eqref{eq:green_diff}, for all $x \in U$ we obtain
\[
    \lim_{\eps\to0} \nabla_i^{(1)}\nabla_j^{(2)} G_{U_\eps}\left(\floor{x/\eps},\floor{x/\eps}\right) = 
    \begin{dcases}
    \hfil \frac12 \ &\text{if} \ i=j \ ,\\
    \frac12 - \frac1\pi \ &\text{if} \ i\neq j \ .
    \end{dcases}
\]
For the case $\floor{x/\eps} - \floor{y/\eps} = (1,0)$ we need to evaluate \eqref{eq:green_double_diff} at $y=x + (1,0)$, which gives
\[
    \nabla_i^{(1)}\nabla_j^{(2)} G_0\left(x,x+(1,0)\right) = 
    \begin{dcases}
    \hfil \frac12 - \frac2\pi \ &\text{if} \ i=1,\, j=1 \ ,\\
    \hfil -1 + \frac2\pi \ &\text{if} \ i=2,\, j=2 \ ,\\
    \hfil -\frac12 + \frac1\pi \ &\text{if} \ i=1,\, j=2 \ ,\\
    \hfil -1 - \frac1\pi \ &\text{if} \ i=2,\, j=1 \ .
    \end{dcases}
\]
Analogously for $\floor{x/\eps} - \floor{y/\eps} = (1,1)$, evaluating at $y = x + (1,1)$ we get
\[
    \nabla_i^{(1)}\nabla_j^{(2)} G_0\left(x,x+(1,1)\right) = 
    \begin{dcases}
    \hfil 0 \ &\text{if} \ i=j \ ,\\
    -1 + \frac3\pi \ &\text{if} \ i\neq j \ .
    \end{dcases}
\]



\marginpar{\textcolor{red}{Correct this once I figure out the previous thing.}}
Finally, \eqref{eq:limit_variance} reads
\begin{equation}\label{eq:conv_less_eps}
    \left[2\pi - 4 \left(1 - \frac1\pi\right)\right] \int_U f(x)^2 \, \d x = \left[2\pi - 4 \left(1 - \frac1\pi\right)\right] \norm{f}_{L^2} \ .
\end{equation}

Let us now analyse the region where $\norm{x-y}\geq\eps$. From Lemma \ref{lemma:bound_2_points_durre}, if $D\subset U$ is a compact set, then $\forall\, x,y \in D_\eps$ we have the bound
\[
   \abs{\nabla_{i,x}\nabla_{j,y}G(x,y)} < c_D \abs{x-y}^{-2}
\]
uniformly in $x$ and $y$, with $c_D$ a constant depending on $D$. Hence, the expectation inside \eqref{eq:variance} for the region $\norm{x-y}\geq\eps$ is a sum of four terms, each of which can be bounded (up to a global constant) by
\[
    \int\displaylimits_{\norm{x-y}\geq\eps} f(x) f(y) \,\eps^4 \,\abs{x-y}^{-4} \d x\, \d y \ .
\]
Although this integral does not have, in general, a simple form solution as in \eqref{eq:conv_less_eps}, under the previous scaling $\eps^{-1}$ a simple change of variables shows that it is finite.

We see then that, for any scaling $\eps^\gamma$ with $\gamma\geq-1$, the variance of $\langle\Phi_\eps,f\rangle$ converges as $\eps\to0$, whereas it diverges for any $\gamma<-1$.

==> cumulants.tex <==
\subsection{Proof of Theorem \ref{thm:cumulants}}\label{subsec:cum}

The strategy to prove the first theorem is based on decomposing the $k$-point functions into combinatorial expressions that involve basically covariances of Gaussian random variables. This is made possible by our explicit knowledge of the Gaussian field which underlies $\Phi_\eps$. These covariances can be estimated using the transfer matrix (Equation \eqref{eq:transfer_cov}), whose scaling limit is well-known: it is the differential of the Laplacian Green's function (cf. \citet[Theorem 1]{kassel-wu}). 


In order to compute the $k$-point function we will first make use of Feynman diagrams techniques, of which we provide a brief exposition in the appendix at the end of the present paper. In particular we will make use of Theorem \ref{thm:janson_general}.

% \begin{theorem}\label{thm:janson}
% Let $Y_\alpha = \,:\!\xi_{\alpha1}\cdots\xi_{\alpha l_\alpha}\!:\,$, where $\{\xi_{\alpha \beta}\}_{1\leq \alpha\leq k, 1\leq \beta\leq l_\alpha}$ are centered jointly normal variables, with $k\geq0$ and $l_1,\dots,l_k\geq0$. Then
% \begin{equation}\label{eq:fd}
%     \E\big[Y_1\cdots Y_k\big] = \sum_\gamma \nu(\gamma) \ ,
% \end{equation}
% where we sum over all \emph{complete} Feynman diagrams $\gamma$ labeled by $\{\xi_{\alpha\beta}\}_{\alpha\beta}$ such that no edge joins two variables $\xi_{\alpha_1\beta_1}$ and $\xi_{\alpha_2\beta_2}$ with $\alpha_1=\alpha_2$.
% \end{theorem}

% The symbol $\nu(\gamma)$ is the so-called \emph{value} of the Feynman diagram $\gamma$. When $\gamma$ is complete, for a collection of vertices $\{\xi_\alpha\}_{1\leq \alpha\leq m}$, $m\in2\N_0$, it is defined as
% \[
%     \nu(\gamma) \coloneqq \prod_{s=1}^{m/2} \E\left[\xi_{\alpha_s}\xi_{\beta_s}\right] \ ,
% \]
% with $\alpha_s,\beta_s\in[m]$, and $\alpha_s \neq \beta_s$ for all $s$.

% The symbol $\nu(\gamma)$ is the so-called \emph{value} of the Feynman diagram $\gamma$, which for a collection of vertices $\{\xi_\alpha\}_{1\leq \alpha\leq m}$, $m\geq0$, is defined as
% \[
%     \nu(\gamma) \coloneqq \prod_{s=1}^r \E\left[\xi_{\alpha_s}\xi_{\beta_s}\right] \prod_{\alpha\in A} \xi_\alpha \ ,
% \]
% with $r \leq m/2$, $\alpha_s,\beta_s\in[m]$, and $\alpha_s \neq \beta_s$ for all $s$. Here, $A$ is the set of unpaired vertices, so that if $\gamma$ is complete, then
% \[
%     \nu(\gamma) = \prod_{s=1}^{m/2} \E\left[\xi_{\alpha_s}\xi_{\beta_s}\right]
% \]
% is a real number ($m$ necessarily needs to be even in order for the diagram to be complete), which is consistent with the fact that \eqref{eq:fd} is an equality between real numbers.
% We refer to \citet[Chapter 1.5]{janson} for an exposition of Feynman diagrams in this context. 

\begin{proof}[Proof of Theorem \ref{thm:cumulants}]
Let us compute the function
\[
    Q_k\big(x^{(1)}_\eps,\dots,x^{(k)}_\eps\big) \coloneqq \E\left[\prod_{j=1}^k{\Phi_\eps\big(x^{(j)}_\eps\big)}\right] \ .
\]
From Definition \ref{def:GradGFF} of $\Phi_\eps\big(x^{(j)}_\eps\big)$ we know that
\[
    Q_k\big(x^{(1)}_\eps,\dots,x^{(k)}_\eps\big) = \sum_{i_1,\dots,i_k\in \mathcal{E}} \E\left[\prod_{j=1}^k:\!\Big(\nabla_{i_j}\Gamma\big(x^{(j)}_\eps\big)\Big)^2\!:\right] \ ,
\]
with $\mathcal E$ the canonical basis of $\R^d$. In our case we have $k$ products of the Wick product $:\!\big(\nabla_{i_j}\Gamma\big(x^{(j)}_\eps\big)\big)^2\!:$ (indexed by $j$, not $i_j$). So we can identify $\xi_{ij}$ in Theorem \ref{thm:janson_general} with $\nabla_{i_j}\Gamma\big(x^{(j)}_\eps\big)$. Since these terms are squared, we need to consider each of them in the product twice.

Let us denote $\overline{x_{e_i}^{(j)}} \coloneqq \big(x^{(j)}, x^{(j)} + e_i\big),\, i\in[d]\,,\, j \in [k]$ (we drop the dependence on $\eps$ to ease notation). Also to make notation lighter we fix the labels $i_j$ for the moment and keep them implicit. We then define $\mathcal{U} \coloneqq \big\{\overline{x^{(1)}},\overline{x^{(1)}},\dots,\overline{x^{(k)}},\overline{x^{(k)}}\big\}$, where each copy is considered distinguishable. We also define $FD_0$ as the set of complete Feynman diagrams on $\mathcal U$ such that no edge joins $\overline{x^{(i)}}$ with (the other copy of) $\overline{x^{(i)}}$. That is, a typical edge $b$ in a Feynman diagram $\gamma$ in $FD_0$ is of the form $\big(\overline{x^{(j)}}, \overline{x^{(m)}}\big)$, with $j\neq m$ and $j,m\in[k]$. Thus by Definition \ref{def:FD} we have
\[
    \E\left[\prod_{j=1}^k:\!\left(\nabla\Gamma\big(x^{(j)}_\eps\big)\right)^2\!:\right] = \sum_{\gamma\in FD_0} \nu(\gamma) = \sum_{\gamma\in FD_0} \prod_{b\in E_\gamma} \E\left[\nabla_{b^+}\Gamma\left((b^+)^-\right)\nabla_{b^-}\Gamma\left((b^-)^-\right)\right] \ ,
\]
where $E_\gamma$ are the edges of $\gamma$ (note that the edges of $\gamma$ connect edges of $U_\eps$) and $(b^+)^-$ denotes the tail of the edge $b^+$ (analogously for $b^-$). Lemma~\ref{lem:grad_gff_cov} and Equation~\eqref{eq:transfer_cov} yield
\[
    \E\left[\prod_{j=1}^k:\!\left(\nabla\Gamma\big(x^{(j)}_\eps\big)\right)^2\!:\right] = \sum_{\gamma\in FD_0} \prod_{b\in E_\gamma} T(b^+,b^-) \ .
\]

Now we would like to express Feynman diagrams in terms of permutations. We first note that any given $\gamma\in FD_0$ cannot join $\overline{x^{(i)}}$ with itself (neither the same nor the other copy of itself). So instead of considering permutations $\sigma\in \mathrm{Perm}(\mathcal U)$ we consider permutations $\sigma'\in S_k$, being $S_k$ the group of permutations of the set $[k]$. Any $\gamma\in FD_0$ is a permutation $\sigma\in \mathrm{Perm}(\mathcal U)$, but given the constraints just mentioned, we can think of them as permutations \mbox{$\sigma'\in S_k$} without fixed points; that is, $\sigma'\in S_k^0$. Thus
\[
    \E\left[\prod_{j=1}^k:\!\left(\nabla\Gamma\big(x^{(j)}_\eps\big)\right)^2\!:\right] = \sum_{\sigma'\in S_k^0} c(\sigma') \prod_{j=1}^k T\left(\overline{x^{(j)}},\overline{x^{(\sigma'(j))}}\right) \ ,
\]
with $c(\sigma')$ a constant that takes into account the multiplicity of different permutations $\sigma$ that give rise to the same $\sigma'$ depending on its number of subcycles, which we will calculate later on.

Let us disassemble this expression even more. In general $\sigma'$ can be decomposed in $q$ cycles. Since $\sigma'\in S_k^0$ (in particular, it has no fixed points), there are at most $\floor{k/2}$ cycles in a given $\sigma'$. Hence,
\[
    \E\left[\prod_{j=1}^k:\!\left(\nabla\Gamma\big(x^{(j)}_\eps\big)\right)^2\!:\right] = \sum_{q=1}^{\floor{k/2}} \sum_{\substack{\sigma'\in S_k^0\\\sigma'=\sigma'_1\dots\sigma'_q}} c(\sigma') \prod_{h=1}^q \prod_{j\in\sigma'_h} T\left(\overline{x^{(j)}},\overline{x^{(\sigma'_h(j))}}\right) \ ,
\]
where the notation $j\in\sigma_h'$ means that $j$ belongs to the domain where $\sigma_h'$ acts (non trivially). Now we note that a cyclic decomposition of a permutation of the set $[k]$ determines a partition $\pi\in\Pi\left([k]\right)$ (although not injectively). This way, a sum over the number of partitions $q$ and $\sigma'\in S_k^0$ with $q$ cycles can be written as a sum over partitions $\pi$ with no singletons, and a sum over full cycles in each block $B$ (that is, those permutations consisting of only one cycle). Hence
\[
    \E\left[\prod_{j=1}^k:\!\left(\nabla\Gamma\big(x^{(j)}_\eps\big)\right)^2\!:\right] = \sum_{\substack{\pi\in\Pi([k])\\\text{\normalfont{w/o singletons}}}} \prod_{B\in\pi} \sum_{\sigma\in S_\mathrm{cycl}(B)} c(\sigma) \prod_{j\in B} T\left(\overline{x^{(j)}},\overline{x^{(\sigma(j))}}\right) \ ,
\]
where we also made the switch between $\prod_{B\in\pi}$ and $\sum_{\sigma\in S_\mathrm{cycl}(B)}$ by grouping by factors. Alternatively, we can express this average in terms of $S_\mathrm{cycl}^0(B)$, the set of full cycles without fixed points, as
\[
    \E\left[\prod_{j=1}^k:\!\left(\nabla\Gamma\big(x^{(j)}_\eps\big)\right)^2\!:\right] = \sum_{\pi\in\Pi([k])} \prod_{B\in\pi} \sum_{\sigma\in S_\mathrm{cycl}^0(B)} c(\sigma) \prod_{j\in B} T\left(\overline{x^{(j)}},\overline{x^{(\sigma(j))}}\right) \ .
\]


As for the multiplicity factor $c(\sigma)$, a straightforward counting calculation shows that it only depends on the size of the partitions $B$, and is equal to
\[
    c(\sigma) = c\left(|B|\right) = 2^{\,\abs{B}-1} \ .
\]
Finally, we need to put back the subscript $i_j$ in the elements $\overline{x^{(j)}}$ and sum over $i_1,\dots,i_k\in \mathcal{E}$. Note that for any function $f:\mathcal E^k \to \R$ we have
\[
    \sum_{i_1,\dots,i_k\in \mathcal{E}} f(i_1,\dots,i_k) = \sum_{\eta:[k]\to\mathcal E} f\left(\eta(1),\dots,\eta(k)\right) \ ,
\]
so that
\[
    \E\left[\prod_{j=1}^k{\Phi_\eps\big(x^{(j)}_\eps\big)}\right] = \sum_{\eta:[k]\to\mathcal E} \sum_{\pi\in\Pi([k])} \prod_{B\in\pi} 2^{\,\abs{B}-1} \sum_{\sigma\in S_\mathrm{cycl}^0(B)} \prod_{j\in B} T\left(\overline{x_{\eta(j)}^{(j)}},\overline{x_{\eta(\sigma(j))}^{(\sigma(j))}}\right) \ ,
\]
and grouping the $\eta(j)$'s according to each block $B\in\pi$ we get
\[
    \E\left[\prod_{j=1}^k{\Phi_\eps\big(x^{(j)}_\eps\big)}\right] =  \sum_{\pi\in\Pi([k])} \prod_{B\in\pi} 2^{\,\abs{B}-1} \sum_{\sigma\in S_\mathrm{cycl}^0(B)} \sum_{\eta:B\to\mathcal E} \prod_{j\in B} T\left(\overline{x_{\eta(j)}^{(j)}},\overline{x_{\eta(\sigma(j))}^{(\sigma(j))}}\right) \ .
\]

Regarding the transfer matrix $T$, using Equation~\eqref{eq:transfer_cov} we can write the above expression as
\[
    \E\left[\prod_{j=1}^k{\Phi_\eps\big(x^{(j)}_\eps\big)}\right] =  \sum_{\pi\in\Pi([k])} \prod_{B\in\pi} 2^{\,\abs{B}-1} \sum_{\sigma\in S_\mathrm{cycl}^0(B)} \sum_{\eta:B\to\mathcal E} \prod_{j\in B} \nabla_{\eta(j)}^{(1)}\nabla_{\eta(\sigma(j))}^{(2)}G_{U_\eps}\big(x^{(j)}_\eps,x^{(\sigma(j))}_\eps\big) \ ,
\]
obtaining the first result of the theorem. Finally, using Lemma~\ref{lemma:conv_green_diff} we obtain the second statement.
\end{proof}



\subsection{Proof of Corollary \ref{cor:cumulants} and Proposition \ref{thm:conformal}}

\begin{proof}[Proof of Corollary \ref{cor:cumulants}]
Recall that Definition~\ref{def:cum_mult} yields
\begin{equation}\label{eq:cum_mom}
    \E\left[\prod_{j=1}^k\Phi_\eps(x_\eps^{(j)})\right] = \sum_{\pi\in\Pi([k])} \prod_{B\in\pi} \kappa\left(\Phi_\eps(x_\eps^{(j)}) : j\in [k]\right) \ .
\end{equation}
The result then follows from expressions \eqref{eq:cumulants} and \eqref{eq:moments_limit} in Theorem \ref{thm:cumulants}.
\end{proof}

The equality in absolute value between our cumulants and those of \citet[Theorem 1]{durre} allow us to adapt his proof and conclude that, in the case of $d=2$, our field is conformally covariant with scale dimension 2.
\begin{proof}[Proof of Proposition \ref{thm:conformal}]
It is known~\cite[Proposition 1.9]{berenotes} that the continuum Green's function $G_U(\cdot, \cdot)$, defined in Equation \eqref{def:cGF}, is conformally invariant against a conformal mapping $h:U\to U'$; that is, for any $v\neq w\in U$,
\[
    G_U(v,w) = G_{U'}\left(h(v),h(w)\right) \ .
\]
Recalling expression \eqref{eq:limiting_cumulants} for the limiting cumulants we see that, for any integer $\ell \geq 2$,
\[
    \lim_{\eps\to 0} \eps^{-2\ell} \kappa\Big(\Phi_\eps\big(x^{(j)}_\eps\big):j\in[\ell]\Big) = 2^{\ell-1}\sum_{\sigma\in S_\mathrm{cycl}^0([\ell])} \sum_{\eta:[\ell]\to\mathcal{E}}\prod_{j=1}^\ell \partial_{\eta(j)}^{(1)}\partial_{\eta(\sigma(j))}^{(2)}G_{U'}\Big(h_\eps\big(x^{(j)}\big), h_\eps\big(x^{(\sigma(j))}\big)\Big) \ .
\]
From the cumulants expression we deduce that, for a given permutation $\sigma$ and assignment $\eta$, each point $x^{(j)}$ will appear exactly twice in the arguments of the product of differences of $G_{U'}$. Thus, using the chain rule and the Cauchy-Riemann equations, for a fixed $\sigma$ we obtain an overall factor $\prod_{j=1}^\ell \big|h'\big(x^{(j)}\big)\big|^2$
after summing over all $\eta$. We then obtain
\[
    \lim_{\eps\to 0} \eps^{-2\ell} \kappa\Big(\Phi_\eps\big(x^{(j)}_\eps\big):j\in[\ell]\Big) = \prod_{j=1}^\ell \abs{h'\big(x^{(j)}\big)}^2 \lim_{\eps\to 0} \eps^{-2\ell} \kappa\Big(\Phi_\eps\Big(h_\eps\big(x^{(j)}\big)\Big):j\in[\ell]\Big) \ .
\]
The result follows plugging this expression into the moments.
\end{proof}

==> discussion.tex <==
\section{Discussion and open questions}\label{sec:dis}

In this paper we studied properties of the gradient squared of the discrete Gaussian free field on $\mathbb{Z}^d$ such as $k$-point correlation functions, cumulants, conformal covariance in $d=2$ and the scaling limit on a domain $U\subset \R^d$. 

One of the most striking result we have obtained is the ``almost'' permanental structure of our field contrasting the block determinantal  structure of the height-one field of the Abelian sandpile studied in \citet{durre, durrethesis,kassel-wu}.
We plan to investigate implications of these structures further in the future. 

%The other direction of research we would like to put forward is the existence of an anomalous scaling for ``squared gradient fields''. It is apparent from the combination of Theorem~\ref{thm:cumulants} and Theorem~\ref{thm:goes_to_WN} that in order to obtain a limit for $\langle \Phi_\eps, \,f\rangle$ one has to ignore the way correlations decay in the gradient squared of the DGFF (namely, like $\eps^{2d}/|v-w|^{2d}$ for $v,\,w$ in the interior of $U$) and rather scale by the {\em sum} of all covariances in $U_\eps$, which is a factor of order $\eps^{d}$. The tightness result implies that this is the only possible non-trivial renormalization of this object. However, we conjecture that by inserting new parameters that make covariances decay more mildly we would obtain a non-trivial limiting object. 

In fact, the idea of the proof for tightness in Proposition \ref{thm:tightness} is based on the application of a criterion by~\citet{mf} for local H\"older and Besov spaces. The proof requires a precise control of the summability of $k$-point functions, which is provided by Theorem~\ref{thm:cumulants} and explicit estimates for double derivatives of the Green's function in a domain. Observe that the proof is based only on the growth of sums of moments at different points. Thus this technique can be generalized to prove tightness of other fields just by having information on these bounds, which is usually easier to obtain than the whole expression on the joint moments.

Regarding the convergence of finite-dimensional distributions, Proposition \ref{prop:convWN}, note that this strategy can be generalized to prove convergence to white noise of other families of fields, given the relatively mild conditions that we used from the field in question. Among them, one only requires knowledge on bounds of sums of joint cumulants, the existence of an infinite volume measure, and the finiteness of the susceptibility constant. Note that similar scaling results were given for random fields on the lattice satisfying the FKG inequality in~\citet{Newman1980Jan}. 



\paragraph*{Acknowledgments}We would like to thank Antal J\'arai for bringing this problem to our attention, sharing his ideas with the authors and for helpful discussions on the topic. We would like to thank the participants of the workshop ``Challenges in Probability and Statistical Mechanics'' at the Technion, Haifa, and G\"unter Last for interesting comments and feedback on this work.

\section*{Funding and data availability statement}
AC initiated this work at TU Delft funded by grant 613.009.102 of the Dutch Organisation for Scientific Research (NWO). RSH was supported by a STAR cluster visitor grant during a visit to TU Delft where part of this work was carried out. AR is supported by Klein-2 grant OCENW.KLEIN.083 and did part of the work at TU Delft.

We do not analyse or generate any datasets, because our work proceeds within a theoretical and mathematical approach.

==> preliminaries.tex <==
\section{Notation and preliminaries}\label{sec:not}

\paragraph{Notation} Let $f,g$ be two functions 
$f,\,g:\, \R^d\to\R^d$, $d\ge 2$.  We will use $f(x)\lesssim g(x)$ to indicate that there exists a constant $C>0$ such that $|f(x)|\le C |g(x)|$, where $|\cdot|$ denotes the Euclidean norm in $\R^d$. If we want to emphasize the dependence of $C$ on some parameter (for example $U$, $\eps$) we will write $\lesssim_U,\,\lesssim_\eps$ and so on. We use the Landau symbol $f=\mathcal O(g)$ if there exist $x_0 \in \R^d,\,C>0$ such that $|f(x)|\le C|g(x)|$ for all $x\ge x_0$. Similarly $f=o(g) $ means that $\lim_{x\to 0}f(x)/g(x)=0$. 
Furthermore, call $[\ell] \coloneqq \{1,\,2,\,\ldots,\,\ell\}$ and $\llbracket-\ell,\ell\rrbracket \coloneqq \{-\ell,\dots,-1,0,1,\dots,\ell\}$, for some $\ell\in \N$. 

We will write $|A|$ for the cardinality of a set $A$. 
For any finite set $A$ we define $\Pi(A)$ as the set of all partitions of $A$. Let $\mathrm{Perm}(A)$ denote the set of all possible permutations of the set $A$ (that is, bijections of $A$ onto itself). When $A = [k]$ for some $k\in\N$, we might also refer to its set of permutations as $S_k$. If we restrict $S_k$ to those permutations without fixed points, we denote them as $S^0_k$.
Call $S_\mathrm{cycl}(A)$ the set of the full cyclic permutations of $A$, possibly with fixed points. More explicitly, any $\sigma:A\to A$ bijective is in $S_\mathrm{cycl}(A)$ if $\sigma(A') \neq A'$ for any subset $A'\subsetneq A$ with $\abs{A'} > 1$. When this condition is relaxed to all $A'$ with $\abs{A'}>0$ we obtain the set of all cyclic permutations without fixed points which is called $S^0_\mathrm{cycl}(A)$. 

\begin{definition}[Cumulants of a random variable]\label{def:cum_single}
Let $X$ be a random variable in $\mathbb{R}^d$ with all moments finite. The cumulant generating function $K(t)$ for $t\in \R^d$ is defined as 
\[
K(t) := \log \left ( \mathbb{E}[e^{ t\cdot X} ]\right ) = \sum_{m=0}^{+\infty} \sum_{m_1+\cdots +m_d=m} \frac{(-1)^m}{m_1!\cdots m_d!} \kappa_m(X) t^{m_1+\cdots + m_d}
\]
where $t\cdot X$ denotes the scalar product in $\R^d$.
The cumulants $(\kappa_m(X))_{m\in\N}$ are obtained from the power series expansion of the cumulant generating function $K(t)$. 
\end{definition}

Let $V=\{v_1,\ldots,\,v_{n}\} $ be a set, $n\in\N$, and $(X_{v_i})_{i=1}^n$ be a family of random variables in $\mathbb{R}^d$ with all finite moments.

\begin{definition}[Joint cumulants of a family of random variables]\label{def:cum_mult}
The joint cumulant generating function $K:\R^d\to \R$ of the family $(X_{v_i})_{i=1}^n$ is defined as
\[
K(t_1,\ldots,\,t_n) := \log \left ( \mathbb{E} \left[e^{\sum_{j=1}^n t_j \cdot X_j} \right ] \right ).
\]
% The joint cumulants are defined as
% \[
% \kappa\left(m_1,\,\ldots,\,m_n\right)=\frac{\partial^{m_1+\cdots+m_n}K(t_1,\ldots,\,t_n)}{\partial^{m_1}t_1\cdots\partial^{m_n}t_n}_{\Big|t_1=\ldots=t_n=0},\quad m_1,\,\ldots,\,m_n\in\N
% \]
The cumulants can be defined as Taylor coefficients of $K(t_1,\ldots,\,t_n)$. The first order (in the Taylor expansion) joint cumulant $\kappa(X_v:\ v\in V)$ of $(X_v)_{v\in V}$ can be computed as 
\[
\kappa(X_v:\ v\in V) := \sum_{\pi \in \Pi(V)} (|\pi|-1)! (-1)^{|\pi|-1} \prod_{B\in \pi} \mathbb{E} \left[\prod_{v\in B} X_v \right].
\]
\end{definition}
Let us remark that by some straightforward combinatorics it follows from the previous definition that
\[
\mathbb{E} \left[\prod_{v\in V} X_v \right] = \sum_{\pi \in \Pi(V)} \prod_{B\in \pi} \kappa(X_v:\ v\in B) \ .
\]
If $V=\{v_1,v_2\}$ then the joint cumulant is the covariance between $X_{v_1}$ and $X_{v_2}$, and if all $n$ random variables are the same then the joint cumulant of the family is equal to $\kappa_n(X)$ in Definition \ref{def:cum_single}.

\subsection{Functions of the Gaussian free field and white noise}\label{sec:GFF} 

Let \mbox{$U\subset\R^d$}, $d\geq 2$, be a non-empty bounded connected open set with smooth boundary. Denote by $(U_{\eps}, E_{\eps})$ the graph with vertex set $U_\eps \coloneqq U/\eps\cap\Z^d$ and edge set $E_\eps$.  For an (oriented) edge $e \in E_{\eps}$ of the graph, we denote by $e^+$ its tip and $e^-$ its tail, and write the edge as $e = (e^-, e^+)$. Consider $\mathcal{E} \coloneqq \{e_i\}_{\,1\leq i\leq d}$, the canonical basis  of $\R^d$. Since we will use approximations via grid points, we need to introduce, for any $t\in \R^d$, its floor function as
\[
    \floor{t} \coloneqq \text{the unique }z\in\Z^d\text{ such that }t\in z+[0,\,1)^d \ .
\]
For any finite set $V \subset \Z^d$ define the {\it discrete (normalized) Laplacian} by
\[
    \Delta_V f(x) \coloneqq \frac{1}{2d}\sum_{y:\,|y-x|=1}\left(f(y)-f(x)\right) \ , \quad f:\Z^d\to\R \ , \ x\in\Z^d \ .
\]

\begin{definition}[Discrete Green's function]\label{def:dGF}
The discrete Green's function in $V$ is the map $G_V:V\times V \to \R$ which is equal to the inverse of $-\Delta_V$ with $0$-boundary conditions, i.e. for fixed $y \in V$
\[
    \begin{dcases}
        \Delta_V G_V(x,y) =- \delta_y(x) \ &\text{if} \  x \in V \ ,\\
        G_V(x,y) = 0 \ &\text{if} \  x\notin V\ ,
    \end{dcases}
\]
where $\delta$ is the Dirac delta function.
\end{definition}

Denote by $G_0(\cdot,\cdot)$ the Green's function for the whole grid $\Z^d$ when $d\geq3$, or with a slight abuse of notation the potential kernel for $d=2$. This abuse of notation is motivated by the fact that we will only be interested in the discrete differences of $G_0$, which exist for the infinite-volume grid in any dimension. Notice that $G_0(\cdot,\cdot)$ is translation invariant; that is, $G_0(v,w) = G_0(0,w-v)$ for all $v,w\in\Z^d$.  
\begin{definition}[Continuum Green's function]\label{def:cGFF}
The {continuum Green's function} $G_U$ on $U \subset \R^d$ is the solution (in the sense of distributions) of 
\begin{equation}\label{def:cGF}
    \begin{dcases}
        \Delta G_U(\cdot, y) = -\delta_y(\cdot) \ &\text{on } U \ ,\\
        G_U(\cdot,y) = 0 \ &\text{on } \partial U \ ,
    \end{dcases}
\end{equation}
for $y\in U$, where $\Delta$ denotes the continuum Laplacian. 
\end{definition}
For an exhaustive treatment on Green's functions we refer to \citet{Evans2010,lawlerlimic} and \citet{spitzer}. 

\begin{definition}[Discrete Gaussian free field, {\citet[Section 2.1]{sznitman2012topics}}]\label{def:dGFF}
Let \mbox{$\Lambda\subset \Z^d$} be finite. The discrete Gaussian free field (DGFF) $(\Gamma(x))_{x\in \Lambda}$ with $0$-boundary condition is defined as the (unique) centered Gaussian field with covariance given by
\[
    \E\left[\Gamma(x) \Gamma(y)\right] = G_\Lambda(x,y) \ , \quad x,y \in \Lambda \ .
\]
\end{definition}
Define for an oriented edge $e = \{e^-, e^+\} \in E_\eps$ the {\it gradient DGFF $\nabla_e\Gamma$} as
\begin{equation}
    \nabla_e\Gamma(e^-) \coloneqq \Gamma(e^+) - \Gamma(e^-) \ .
\end{equation}
In the following, we will define the main object of interest.

\begin{definition}[Gradient squared of the DGFF]\label{def:GradGFF}
The discrete stochastic field $\Phi_\eps$ given by
\[
   \Phi_\eps(x) \coloneqq \sum_{i=1}^d{:\!\left({\nabla_{e_i}\Gamma}(x)\right)^2\!:} \ , \quad x \in U_\eps \ ,
\]
is called the gradient squared of the DGFF, where $: \ :$ denotes the Wick product; that is, $:\!X\!:\, = X - \E[X]$ for any random variable $X$.
\end{definition}

The family of random fields $\left(\Phi_\eps\right)_{\eps>0}$ is a family of distributions, which acts on a given test function $f\in\mathcal C_c^\infty(U)$ as
\begin{equation}\label{def:action}
    \langle\Phi_\eps,f\rangle = \int_U {\Phi_\eps\left(\floor{x/\eps}\right) f(x) \, \d x} \ ,
\end{equation}
where $\langle \cdot, \cdot \rangle$ denotes the scalar product in $L^2(U)$.


When no ambiguities appear, we will write $\left(\nabla_i\Gamma(x)\right)^2$ for $\left(\nabla_{e_i}\Gamma(x)\right)^2$, with $i=1,2,\dots,d$. 
For any given function $f:\Z^d\times\Z^d\to\R$, we define the {\it discrete gradient} in the first argument and direction $e_i\in\mathcal E$ as
\[
    \nabla_{e_i}^{(1)}f(x,y) \coloneqq f(x+e_i,y) - f(x,y) ,
\]
with $x,y\in\Z^d$, and analogously
\[
    \nabla_{e_i}^{(2)}f(x,y) \coloneqq f(x,y+e_i) - f(x,y)
\]
for the second argument. Once again, when no ambiguities arise, we will write $\nabla_i^{(1)}$ for $\nabla_{e_i}^{(1)}$, and analogously for the second argument. 

For a continuum function $g:U\times U\to\R$, $\partial_{e_i}^{(1)}g(x,y)$ denotes the partial derivative of $g$ with respect to the first argument in the direction of $e_i$, while $\partial_{e_i}^{(2)}g(x,y)$ corresponds to the second argument, also in the direction $e_i$. The same abuse of notation on the subindex $e_i$ applies here.

\begin{definition}[Gaussian white noise]\label{def:WN}
The $d$-dimensional Gaussian white noise $W$ is the centered Gaussian random distribution on $U \subset \R^d$ such that, for every $f,g\in L^2(U)$, 
\[
\mathbb{E}\left[\langle W,f \rangle \langle W,g \rangle\right] = \int_{U\times U} f(x) g(x) \d x  \ .
\]
In other words, $\langle W,f \rangle \sim \mathcal N \big(0, \|f\|^2_{L^2(U)} \big)$ for every $f\in L^2(U)$. 
\end{definition}

\subsection{Besov-H\"older spaces}

In this Subsection we will define the functional space on which convergence will take place. We will use \citet{mf} as a main reference. Local H\"older and Besov spaces of negative regularity on general domains are natural functional spaces when considering scaling limits of certain random distributions or in the context of non-linear stochastic PDE's, see e.g. \citet{mf,Hairer} especially when those objects are well-defined on a domain $U \subset \R^d$ but not necessarily on the full space $\R^d$. They are particularly suited for fields which show bad behaviour near the boundary $\partial U$.

Let $(V_n)_{n\in \mathbb{Z}}$ be a dense subsequence of subspaces of $L^2(\R^d)$ such that $\bigcap_{n\in \mathbb{Z}} V_n = \{0\}$. Denote by $W_n$ the orthogonal complement of $V_n$ in $V_{n+1}$ for all $n\in \mathbb{Z}$. Furthermore, we assume the following properties. The function $f\in V_n$ if and only if $f(2^{-n} \cdot) \in V_0$. Let $(\phi(\cdot -k))_{k\in \mathbb{Z}^d}$ be an orthonormal basis of $V_0$ and $(\psi^{(i)}(\cdot -k))_{i<2^d, k\in \mathbb{Z}^d}$ an orthonormal basis of $W_0$. Note that $\phi, (\psi^{(i)})_{i<2^d}$ both belong to $\mathcal{C}^r_c(\R^d)$ for some positive integer $r \in \mathbb{N}$, that is, they belong to the set of $r$ times continuously differentiable functions on $\R^d$ with compact support.

Define moreover $\Lambda_n=\mathbb{Z}^d/2^n$ and
\[
\phi_{n,x}(y) = 2^{dn/2}\phi\big(2^n(y-x)\big)
\]
resp.
\[
\psi^{(i)}_{n,x}(y) = 2^{dn/2}\psi^{(i)}\big(2^n(y-x)\big)
\]
which makes $(\phi_{n,x})_{x\in \Lambda_n}$ an orthonormal basis of $V_n$ resp. $(\psi^{(i)}_{n,x})_{x\in \Lambda_n, i<2^d, n\in \mathbb{Z}}$ an orthonormal basis of $L^2(\R^d)$. Every function $f\in L^2(\R^d)$ can be decomposed into
\[
f = \mathcal{V}_k f + \sum_{n=k}^{\infty} \mathcal{W}_n f
\]
for any fixed $k\in \mathbb{Z}$, where $\mathcal{V}_k$ resp. $\mathcal{W}_k$ are the orthogonal projections of $V_n$ resp. $W_n$ defined as
\[
\mathcal{V}_n f = \sum_{x\in \Lambda_n} \big\langle f,\phi_{n,x}\big\rangle \phi_{n,x} \ , \quad \mathcal{W}_n f = \sum_{i<2^d, x\in \Lambda_n} \big\langle f,\psi^{(i)}_{n,x}\big\rangle \psi^{(i)}_{n,x} \ .
\]

\begin{definition}[Besov spaces]\label{def:locBes}
Let $\alpha \in \R$, $|\alpha|<r$, $p,q\in [1,\infty]$ and $U\subset \R^d$. The Besov space $\mathcal{B}^{\alpha}_{p,q}(U)$ is the completion of $\mathcal{C}^{\infty}_c(U)$ with respect to the norm
\[
\|f\|_{\mathcal{B}^{\alpha}_{p,q}} \coloneqq \|\mathcal{V}_0 f\|_{L^p} + \left\| \big(2^{\alpha n} \|\mathcal{W}_n f\|_{L^p}\big)_{n\in \mathbb{N}}\right\|_{\ell^q} \ .
\]
The local Besov space $\mathcal{B}^{\alpha, \mathrm{loc}}_{p,q}(U)$ is the completion of $\mathcal{C}^{\infty}(U)$ with respect to the family of semi-norms
\[
f \mapsto \| \widetilde\chi f\|_{\mathcal{B}^{\alpha}_{p,q}}
\]
indexed by $\widetilde\chi \in \mathcal{C}^{\infty}_c(U)$.
\end{definition}


We will use the following embedding property of Besov spaces in the tightness argument.

\begin{lemma}[{\citet[Remark 2.12]{mf}}]\label{lemma:embedding}
    For any $1\leq p_1 \leq p_2 \leq\infty$, $q\in[1,\infty]$ and $\alpha\in\R$, the space $\mathcal B_{p_2,q}^{\alpha,\mathrm{loc}}(U)$ is continuously embedded in $\mathcal B_{p_1,q}^{\alpha,\mathrm{loc}}(U)$.
\end{lemma}

Finally let us define the functional space where convergence will take place, the space of distributions with locally $\alpha$-H\"older regularity.

\begin{definition}[H\"older spaces]\label{def:locHoel}
Let $\alpha < 0,r_0=-\lfloor \alpha \rfloor$. The space $\mathcal C^{\alpha}_{\mathrm{loc}}(U)$ is called the locally H\"older space with regularity $\alpha \in \R$ on the domain $U$. It is the completion of $\mathcal{C}^{\infty}_c(U)$ with respect to the family of semi-norms
\[
f \mapsto \|\widetilde\chi f\|_{\mathcal{C}^{\alpha}}
\]
indexed by $\widetilde\chi \in \mathcal{C}^{\infty}_c(U)$ and
\[
\| f\|_{\mathcal C_{\alpha}} = \sup_{\lambda \in (0,1]} \sup_{x\in \R^d} \sup_{\eta \in B^{r_0}} \lambda^{-\alpha} \int_{\R^d} f(\cdot) \, \lambda^{-d} \,\eta\left(\frac{\cdot -x}{\lambda}\right) \ ,
\]
where
\[
B^{r_0} = \left\{ \eta \in \mathcal C^{r_0}:\|\eta \|_{\mathcal C^{r_0}} \leq 1, \, \supp \eta \subset B(0,1) \right\} \ .
\]
\end{definition}

Note that by \citet[Remark 2.18]{mf} one has $\mathcal C^{\alpha}_{\mathrm{loc}}(U) = \mathcal{B}^{\alpha, \mathrm{loc}}_{\infty,\infty}(U)$.

==> previous_results.tex <==
\section{Proofs}\label{sec:proofs}

\subsection{Previous results from literature}

Let us now expose some important results that we will refer to throughout the proofs. They refer to partially known results and partially consist of straightforward generalizations of previous results.

Our computations will rely on the fact that the distribution of the gradient field $\nabla_i \Gamma$, \mbox{$i\in [d]$}, is well-known. The following result is quoted from \citet[Lemma 3.6]{funaki}.

\begin{lemma}\label{lem:grad_gff_cov}
Let \mbox{$\Lambda\subset \Z^d$} be finite, and let $(\Gamma_x)_{x\in \Lambda}$ be a $0$-boundary conditions DGFF on $\Lambda$ (see Definition \ref{def:dGFF}). Then
\[
\begin{dcases}
\E\left[\nabla_i \Gamma(x)\right]=0 \ &\text{if} \ x\in\Lambda\ , \ i\in[d] \ , \\
    \E\left[\nabla_i \Gamma(x)\nabla_j \Gamma(y)\right]=\nabla^{(1)}_i\nabla^{(2)}_j G_\Lambda(x,\,y) \ &\text{if} \ x,\,y\in\Lambda \ ,\ i,\,j\in[d] \ .
\end{dcases}
\]
\end{lemma}
Consequently, we can directly link the gradient DGFF to so-called  transfer current matrix $T(\cdot,\cdot)$ by
\begin{equation}
    T(e,f) = G_\Lambda(e^-,f^-)-G_\Lambda(e^+,f^-)-G_\Lambda(e^-,f^+)+G_\Lambda(e^+,f^+)
\end{equation}
where $e,\,f$ are oriented edges of $\Lambda$ (see \citet[Section 2]{kassel-wu}). Equivalently we can write
\begin{equation}\label{eq:transfer_cov}
    T(e,f) = \nabla_e\nabla_f G_\Lambda(e^-,f^-) \ .
\end{equation}

From Lemma~\ref{lem:grad_gff_cov}, it is clear that we need to control the behaviour of double derivatives of discrete Green's function in the limit $\varepsilon\to 0$. In order to find the limiting joint moments of the point-wise field $\Phi_\eps(x)$ we will need the following result about the convergence of the discrete difference of the Green's function on $U_\eps$ (see Definition \ref{def:dGF}) to the double derivative of the continuum Green's function $G_U(\cdot,\cdot)$ on a set $U$ (see Equation \eqref{def:cGF}). This result follows from Theorem 1 of \citet{kassel-wu}.

\begin{lemma}[\textit{Convergence of the Green's function differences}]\label{lemma:conv_green_diff}
    Let $v$, $w$ be points in the set $U$, with $v \neq w$. Then for all $a,b \in \mathcal E$,
    \[
       \lim_{\eps\to 0} \eps^{-d}\, \nabla_{a}^{(1)}\nabla_{b}^{(2)}G_{U_\eps}\left(\floor{v/\eps},\floor{w/\eps}\right) = \partial_{a}^{(1)}\partial_{b}^{(2)}G_U(v,w) \ .
    \]
\end{lemma}

The next lemma is a generalization of \citet[Lemma 31]{durrethesis} for general dimensions $d\geq 2$. The proof is straightforward and will be omitted.
It provides an error estimate when replacing the double difference of $G_{U_\eps}(\cdot,\cdot)$ on the finite set by that of $G_0(\cdot,\cdot)$ defined on the whole lattice. 

\begin{lemma}\label{lemma:bound_2_points_durre}
    Let $D\subset U$ be such that the distance between $D$ and $U$ is non-vanishing, that is, $\dist{(D,\partial U)} \coloneqq \inf_{(x,y)\in D\times\partial U}\abs{x-y} > 0$. There exist $c_D > 0$ and $\eps_D > 0$ such that, for all $\eps \in (0,\eps_D]$, for all $v,w \in D_\eps \coloneqq D/\eps \cap \Z^d$ and $i,j\in[d]$,
    \begin{equation}\label{eq:one_durre}
        \abs{\nabla_i^{(1)}\nabla_j^{(2)} G_{U_\eps}(v,w) - \nabla_i^{(1)}\nabla_j^{(2)} G_0(v,w)} \leq c_D \, \eps^d \ ,
    \end{equation}
    and also
    \begin{equation}\label{eq:two_durre}
      \abs{\nabla_i^{(1)}\nabla_j^{(2)} G_{U_\eps}(v,w)} \leq c_D \cdot
        \begin{dcases}
            \ \abs{v-w}^{-d} \ &\text{if} \ v\neq w \ ,\\
            \hfil 1 \ &\text{if} \ v = w \ .
        \end{dcases}
    \end{equation}
\end{lemma}

An immediate consequence of \eqref{eq:two_durre} and the expression \eqref{eq:cumulants} in Theorem \ref{thm:cumulants} for two points gives us the following bound on the covariance of the field:

\begin{corollary}\label{cor:covariance_bound}
    Let $D$, $v$ and $w$ be as in Lemma \ref{lemma:bound_2_points_durre}. Then
    \begin{equation}\label{eq:bound_double_diff}
        \E\left[\Phi_\eps(v)\Phi_\eps(w)\right] \leq c_D \cdot
        \begin{dcases}
            \abs{v-w}^{-2d} \ &\text{if} \ v\neq w \ ,\\
            1 \ &\text{if} \ v = w \ .
        \end{dcases}
    \end{equation}
\end{corollary}

On the other hand, we will also make use of a straightforward extension of~\citet[Corollary 4.4.5]{lawlerlimic} for $d=2$ and \citet[Corollary 4.3.3]{lawlerlimic} for $d\geq 3$, yielding the following Lemma.

\begin{lemma}[Asymptotic expansion of the Green's function differences]\label{lemma:lemma_29_durre}
As $|v|\to+\infty$, for all $i,\,j\in[d]$
\[
    \abs{\nabla_i^{(1)}\nabla_j^{(2)} G_{0}(0,v)}=\mathcal O\big(|v|^{-d}\big) \ .
\]
\end{lemma}

The following technical combinatorial estimate, which is an immediate extension of a corollary of \citet[Lemma 37]{durrethesis}, will be important when proving tightness of the family $(\Phi_\eps)_\eps$, in order to bound the rate of growth of the moments of $\langle\Phi_\eps,f\rangle$ for some test function $f$:

\begin{lemma}\label{lemma:sum_p_point_function}
    Let $D \subset U$ such that $\dist{(D,\partial U)} > 0$ and $p\geq2$. Then
    \[
        \sum_{\substack{v_1,\dots,v_p\in D_\eps\\v_i\neq v_j \mathrm{ for }\, i\neq j}} \left(\prod_{i=1}^{p-1} \frac{1}{\left|v_i-v_{i+1}\right|^d}\right) \frac{1}{\left|v_p-v_1\right|^d} = \mathcal O_{D}\left(\eps^{-\frac{p}{2}-d+1}\right) \ ,
    \]
    where $D_\eps \coloneqq D/\eps\cap\Z^d$.
\end{lemma}



==> results.tex <==
\section{Main results}\label{sec:main}

The first result we would like to present is an explicit computation of the $k$-point correlation function of the  gradient squared of the DGFF field $\Phi_\eps$ defined in Definition \ref{def:GradGFF}.

\begin{theorem}\label{thm:cumulants}
Let $\eps>0$ and $k \in \mathbb{N}$ and let the points $x^{(1)},\dots,x^{(k)}$ in $U \subset \R^d$, $d\geq 2$, be given. Define $x^{(j)}_\eps \coloneqq \floor{x^{(j)}/\eps}$ so that $x^{(j)}_\eps \in U_\eps$, for $j = 1,\dots,k$. Then
\begin{equation}\label{eq:cumulants}
    \E\left[\prod_{j=1}^k{\Phi_\eps\big(x^{(j)}_\eps\big)}\right] = \sum_{\pi\in\Pi([k])}\prod_{B\in\pi}2^{|B|-1}\sum_{\sigma\in S_\mathrm{cycl}^0(B)} \sum_{\eta:B\to\mathcal{E}}\prod_{j\in B} \nabla_{\eta(j)}^{(1)}\nabla_{\eta(\sigma(j))}^{(2)}G_{U_\eps}\big(x^{(j)}_\eps,x^{(\sigma(j))}_\eps\big) \,
\end{equation}
where $G_{U_{\eps}}(\cdot,\cdot)$ was defined in Definition \ref{def:dGF}.
Moreover if $x^{(i)} \neq x^{(j)}$ for all $i \neq j$, then
\begin{multline}\label{eq:moments_limit}
    \lim_{\eps\to 0} \eps^{-dk}\E\left[\prod_{j=1}^k{\Phi_\eps\big(x^{(j)}_\eps\big)}\right] = \sum_{\pi\in\Pi([k])}\prod_{B\in\pi}2^{|B|-1}
    \sum_{\sigma\in S_\mathrm{cycl}^0(B)} \\
    \sum_{\eta:B\to\mathcal{E}}\prod_{j\in B} \partial_{\eta(j)}^{(1)}\partial_{\eta(\sigma(j))}^{(2)}G_U \big(x^{(j)}, x^{(\sigma(j))}\big) \,
\end{multline}
where $G_U(\cdot,\cdot)$ was defined in Equation \eqref{def:cGF}.
\end{theorem}

\begin{remark}
    It will sometimes be useful to write \eqref{eq:cumulants} as the equivalent expression
    \begin{equation}\label{eq:cumulants2}
        \E\left[\prod_{j=1}^k{\Phi_\eps\big(x^{(j)}_\eps\big)}\right] = \sum_{\substack{\pi\in\Pi([k])\\\text{\normalfont{w/o singletons}}}} \prod_{B\in\pi}2^{|B|-1}\sum_{\sigma\in S_\mathrm{cycl}(B)} \sum_{\eta:B\to\mathcal{E}}\prod_{j\in B} \nabla_{\eta(j)}^{(1)}\nabla_{\eta(\sigma(j))}^{(2)}G_{U_\eps}\big(x^{(j)}_\eps,x^{(\sigma(j))}_\eps\big) \ ,
    \end{equation}
    where the condition of $\sigma$ belonging to full cycles of $B$ without fixed points is inserted in the no-singleton condition of the permutations $\pi$.
\end{remark}

\begin{remark}
    From the above expression it is immediate to see that the $2$-point function is given by
    \[
        \E\left[\Phi_\eps\big(x_\eps\big) \Phi_\eps\big(y_\eps\big)\right] =2\sum_{i,j\in[d]} \left(\nabla_i^{(1)}\nabla_j^{(2)}G_{U_\eps}\big(x_\eps,y_\eps\big)\right)^2 \ ,
    \]
    which will be useful later on.
\end{remark}


The following Corollary is a direct consequence of Theorem \ref{thm:cumulants}.

\begin{corollary}\label{cor:cumulants}
Let $\ell\in\N$. The joint cumulants $\kappa\left(\Phi_\eps\big(x^{(j)}_\eps\big):j\in[\ell],\,x^{(j)}_\eps\in U_\eps\right)$ of the field $\Phi_{\eps}$ at ``level'' $\eps>0$ are given by
\begin{equation}\label{eq:cumulants3}
    \kappa\Big(\Phi_\eps\big(x^{(j)}_\eps\big):j\in[\ell]\Big) = 2^{\ell-1}\sum_{\sigma\in S_\mathrm{cycl}^0([\ell])} \sum_{\eta:[\ell]\to\mathcal{E}}\prod_{j=1}^\ell \nabla_{\eta(j)}^{(1)}\nabla_{\eta(\sigma(j))}^{(2)}G_{U_\eps}\big(x^{(j)}_\eps,x^{(\sigma(j))}_\eps\big) \ .
\end{equation}
Moreover if $x^{(i)} \neq x^{(j)}$ for all $i \neq j$, then
\begin{equation}\label{eq:limiting_cumulants}
    \lim_{\eps\to 0} \eps^{-d\ell} \kappa\Big(\Phi_\eps\big(x^{(j)}_\eps\big):j\in[\ell]\Big) = 2^{\ell-1}\sum_{\sigma\in S_\mathrm{cycl}^0([\ell])} \sum_{\eta:[\ell]\to\mathcal{E}}\prod_{j=1}^\ell \partial_{\eta(j)}^{(1)}\partial_{\eta(\sigma(j))}^{(2)}G_U\big(x^{(j)},x^{(\sigma(j))}\big) \ .
\end{equation}
\end{corollary}
As already mentioned in the introduction, comparing our result with~\citet[Theorem 2]{durre} we obtain~\eqref{eq:equal_cumulants}.
 
The following proposition states that in $d=2$ the limit of the field $\Phi_{\eps}$ is conformally covariant with scale dimension 2. This result can also be deduced for the height-one field for the sandpile model, see \citet[Theorem 1]{durre}.

\begin{prop}\label{thm:conformal}
    Let $U,U' \subset \R^2$, $k\in \mathbb{N}$, $\big\{x^{(j)}\big\}_{j\in[k]}$, and $\big\{x^{(j)}_\eps\big\}_{j\in[k]}$ be as in Theorem \ref{thm:cumulants}. Furthermore let $h:U\to U'$ be a conformal mapping and call $h_\eps\big(x^{(j)}\big) \coloneqq \floor{h\big(x^{(j)}\big)/\eps}$. Then
    \[
        \lim_{\eps\to 0} \eps^{-2k}\E\left[\prod_{j=1}^k{\Phi_\eps\big(x^{(j)}_\eps\big)}\right] = \prod_{j=1}^k \abs{h'\big(x^{(j)}\big)}^2 \lim_{\eps\to 0} \eps^{-2k}\E\left[\prod_{j=1}^k{\Phi_\eps\Big(h_\eps\big(x^{(j)}\big)\Big)}\right] \ .
    \]
\end{prop}
% Let us now show in which sense we can make our field converge to white noise. First of all, we way in which we previously defined the action $\langle\Phi_\eps,f\rangle$ on a given test function $f$ was \textcolor{red}{(say where I defined this (once I do it))}
% \[
%     \langle\Phi_\eps,f\rangle = \int_U {\Phi_\eps\left(\floor{x/\eps}\right) f(x) \, \d x} .
% \]
% For the sake of convenience of computations, we will define $\left\langle\Phi_\eps,f\right\rangle$ as
% \[
%     \langle \Phi_\eps,f\rangle = \sum_{v\in U_\eps} {f(\eps v)\Phi_\eps(v)} .
% \]
% \textcolor{red}{Write explicitly the computation that shows that the difference of both of this expressions is $\mathcal O(\eps^2)$. IMPORTANT: for it to be $\mathcal O(\eps^2)$, the integral should have scaling $\eps^{-1}$, and the sum $\eps$.}

% \marginpar{Write only ONE def of <,> (the integral probably). In the proof of thm 3, write a lemma first, saying that this def in integral form is equal to the sum def, up to eps2.}

Finally we will show that the rescaled gradient squared of the discrete Gaussian free field will converge to white noise in some appropriate locally H\"older space with negative regularity $\alpha$ in $d\geq 2$ dimensions. This space is denoted as $\mathcal C_\mathrm{loc}^\alpha(U)$ (see Definition \ref{def:locHoel}).


\begin{theorem}\label{thm:goes_to_WN}
    Let $U\subset \R^d$ with $d\geq 2$. The gradient squared of the discrete Gaussian free field $\Phi_{\eps}$ converges in the following sense as $\eps\to0$:
    \[
        \frac{\eps^{-d/2}}{\sqrt \chi} \Phi_{\eps} \overset{d}\longrightarrow W,
    \]
    where the white noise $W$ is defined in Definition \ref{def:WN}.
    This convergence takes place in $\mathcal C^{\alpha}_{\mathrm{loc}}(U)$ for any $\alpha < -d/2$, and the constant $\chi$ defined as
    \begin{equation}\label{eq:chi_def}
        \chi \coloneqq 2\sum_{v\in\Z^d} \sum_{i,j\in[d]} \left(\nabla_i^{(1)}\nabla_j^{(2)}G_0(0,v)\right)^2
    \end{equation}
    is well-defined, in the sense that $0<\chi<\infty$.
\end{theorem}

\begin{remark}
Let us remind the reader that $\mathcal C^{\alpha}_{\mathrm{loc}}(U)$ with $\alpha < -d/2$ are the optimal spaces in which the white noise lives. See for example \citet[Proposition 5.9]{mourratarmstrong}.
\end{remark}

%%%%%%%%%%

\subsection{Fock space structure}\label{subsec:fock}

Let us discuss in the following the connection to Fock spaces. We start by reminding the reader of the definition of the continuum Gaussian free field (GFF).

\begin{definition}[Continuum Gaussian free field, {\citet[Section 1.5]{berenotes}}]
The continuum Gaussian free field $\overline{\Gamma}$ with $0$-boundary (or Dirichlet) conditions outside $U$ is the unique centered Gaussian process indexed by $C_c^\infty(U)$ such that
\[
    \cov{\big(\overline{\Gamma}(f),\overline{\Gamma}(g)\big)} = \int_{U\times U} f(x)g(y)G_U(x,\,y) \, \d x\d y \ , \quad f,\,g\in C_c^\infty(U)\ , 
\]
where $G_U(\cdot, \cdot)$ was defined in Definition \ref{def:cGFF}.
\end{definition}

We can think of it as an isometry $\overline{\Gamma}: \mathcal H \to L^2(\Omega,\mathbb P)$, for some Hilbert space $\mathcal H$ and some probability space $(\Omega, \mathcal{F},\mathbb P)$. To fix ideas, throughout this Section let us fix $\mathcal H\coloneqq\mathcal H_0^1(U)$, the order one Sobolev space with Dirichlet inner product (see~\citet[Section 1.6]{berenotes}). Note that, even if the GFF is not a proper random variable, we can define its derivative as a Gaussian distributional field.
\begin{definition}[Derivatives of the GFF,~{\citet[pg. 4]{kang2013gaussian}}]
The derivative of $\overline{\Gamma}$ is defined as the Gaussian distributional field $\partial_i \overline{\Gamma}$, $1\le i\le d$, in the following sense:
\[
\big(\partial_i \overline{\Gamma}\big)(f)\coloneqq \overline{\Gamma}\left(\partial_i f\right) \ ,\quad f\in C_c^\infty(U) \ .
\]
\end{definition}
There is however another viewpoint that one can take on the GFF and its derivatives, and is that of viewing them as {\em Fock space fields}. This approach will be used to reinterpret the meaning of Theorem~\ref{thm:cumulants}. For the reader's convenience we now recall here some basic facts about Fock spaces and their fields. Our presentation is drawn from~\citet[Section 3.1]{janson} and~\citet[Sec. 1.2-1.4]{kang2013gaussian}.

For $n\geq0$, we denote $\mathcal H^{\odot n}$ as the $n$-th symmetric tensor power of $\mathcal H$; in other words, $\mathcal H^{\odot n}$ is the completion of linear combinations of elements $f_1\odot\cdots\odot f_n$ with respect to the inner product 
\[
    \left\langle f_1\odot\cdots\odot f_n, g_1\odot\cdots\odot g_n \right\rangle = \sum_{\sigma\in S_n} \prod_{i=1}^n \big\langle f_i,g_{\sigma(i)}\big\rangle \ ,\quad f_i,\, g_i\in \mathcal H \ ,\ 1\le i\le n \ .
\]
The symmetric Fock space over $\mathcal H$ is
\[
    \mathrm{Fock}(\mathcal H) \coloneqq \bigoplus_{n\geq0} \mathcal{H}^{\odot n} \ .
\]

% This way, the product operation $\odot$ of the algebra $\sum_{n\geq0}\mathcal H^{\odot n}$ corresponds to a  projection given by
% \[
%     asdf
% \]


% for $X\in\mathcal H_p$, $Y\in\mathcal H_q$, where
% \[
%     \mathcal H_p \coloneqq  \ .
% \]
% We call it \emph{Wick product}, and denote it also as $:XY:$\,.
We now introduce elements in $Fock(\mathcal H)$ called {\em Fock space fields}. We call \emph{basic correlation functionals} the formal expressions of the form
\[
    \mathcal X_p = X_{1}(x_{1})\odot\cdots\odot X_{p}(x_{p}) \ ,
\]
for $p\in\N$, $x_{1},\dots,x_{p}\in U$, and $X_{1},\dots,X_{p}$ derivatives of $\overline \Gamma$. The set $\mathcal S(\mathcal X_p)\coloneqq\{x_1,\,\ldots,\,x_p\}$ is called the set of {\em nodes} of $\mathcal X_p$. Basic Fock space fields are formal expressions written as products of
derivatives of the Gaussian free field $\overline \Gamma$, for example $1\odot \overline\Gamma$, $\partial \overline\Gamma\odot\overline\Gamma\odot \overline\Gamma $ etc. A general Fock space field $X$ is a linear combination of basic fields. We think of any such $X$ as a map $u\mapsto X(u)$, $u\in U$, where the values $\mathcal X=X(u)$ are correlation functionals with $\mathcal S(\mathcal X)=\{u\}$. Thus Fock space fields are functional-valued functions. Observe that Fock space fields may or may not be distributional random fields, but in any case we can think of them as functions in $U$ whose
values are correlation functionals.

Our goal is to define now tensor products. We will restrict our attention to tensor products over an even number of correlation functionals, even if the definition can be given for an arbitrary number of them. The reason behind this presentation is due to the set-up we will be working with.
\begin{definition}[Tensor products in Fock spaces]
Let $m\in 2\N$. Given a collection of correlation functionals 
\[\mathcal X_j\coloneqq X_{j1}(z_{j1})\odot \cdots \odot X_{j n_j}(z_{j n_j}) \ ,\quad 1\le j\le m
\]
with pairwise disjoint $\mathcal S(\mathcal X_j)$'s, the tensor product of the elements $\mathcal X_1,\ldots,\mathcal X_m$ is defined as
\begin{equation}\label{eq:tensor}
    \mathcal X_1 \cdots \mathcal X_m \coloneqq \sum_\gamma \prod_{\{u,v\}\in E_\gamma} \E\left[X_u(x_u)X_v(x_v)\right] \ ,
\end{equation}
where the sum is taken over Feynman diagrams $\gamma$ with vertices $u$ labeled by functionals $X_{pq}$ in such a way that there are no contractions of vertices in the same $\mathcal S(\mathcal X_p)$. $E_\gamma$ denotes the set of edges of $\gamma$. One extends the definition of tensor product to general correlation functionals by linearity.
\end{definition}


The reader may have noticed that~\eqref{eq:tensor} is simply one version of Wick's theorem. It is indeed this formula that will allow us in Subsection~\ref{subsec:cum} to prove Theorem~\ref{thm:cumulants}, and that enables one to bridge Fock spaces and our cumulants in the following way.  For any $j\in[k]$, $k\in\N$, $i_j\in[d]$ and $x^{(j)}\in U$ one can define the basic Fock space field $X_{i_j}\big(x^{(j)}\big)\coloneqq\partial_{i_j} \overline{\Gamma}\big(x^{(j)}\big)$. Introduce the correlation functional 
\begin{equation}\label{eq:Y}
    \mathcal Y_j\coloneqq\sum_{i_j\in \mathcal E}X_{i_j}^{\odot 2}\big(x^{(j)}\big) \ .
\end{equation}
We obtain now the statement of the next Lemma.
\begin{lemma}[$k$-point correlation functions as Fock space fields] Under the assumptions of Theorem~\ref{thm:cumulants},
\[
  \lim_{\eps\to 0} \eps^{-dk}\E\left[\prod_{j=1}^k{\Phi_\eps\big(x^{(j)
  }_\eps\big)}\right] = \sum_{\pi\in \Pi[k]}2^{k-|\pi|}\prod_{B\in \pi}\mathcal Y_B\big(x^{(B)}\big)
  \]
  where ${\mathcal Y}_B\big(x^{(B)}\big)\coloneqq{\mathcal Y}_1\big(x^{(1)}\big)\odot\cdots\odot{\mathcal Y}_j\big(x^{(j)}\big),\,j\in B$. Here $|\pi|$ stands for the number of blocks of the partition $\pi$.
\end{lemma}
%One can see that the right-hand side of~\eqref{eq:moments_limit} is nothing but the tensor product $\mathcal Y_1\cdots\mathcal Y_k$ of correlation functionals. 
The Fock space structure is more evident from the Gaussian perspective of the DGFF, but~\eqref{eq:equal_cumulants} together with D\"urre's theorem entail a corollary which we would like to highlight. We remind the reader of the definition of the constant $C$ in~\eqref{eq:def_C}.
\begin{corollary}[Height-one field $k$-point functions, $d=2$]\label{cor:cum_in_height}
With the same notation of Theorem~\ref{thm:cumulants} one has in $d=2$ that
\[\lim_{\eps\to 0} \eps^{-2k} \mathbb E\left[\prod_{j=1}^k{\left(h_\eps\big(x^{(j)}_\eps\big)-\mathbb E\left[h_\eps\big(x^{(j)}_\eps\big)\right]\right)}\right] =\sum_{\pi\in \Pi[k]}(-2)^{|\pi|}\prod_{B\in \pi}\widetilde{\mathcal Y}_B\big(x^{(B)}\big)
\]
where $\widetilde{\mathcal Y}_B\big(x^{(B)}\big)\coloneqq\widetilde{\mathcal Y}_1\big(x^{(1)}\big)\odot\cdots\odot\widetilde{\mathcal Y}_j\big(x^{(j)}\big),\,j\in B$ and $\widetilde{\mathcal Y}_j\coloneqq C/2\,\mathcal Y_j$. As before, $|\pi|$ stands for the number of blocks of the partition $\pi$.
\end{corollary}




==> tightness2.tex <==
\subsection{Proof of Theorem \ref{thm:goes_to_WN}}

The proof of this Theorem will be split into two parts. First we will show that the family $(\Phi_\eps)_{\eps>0}$ is tight in some appropriate Besov space and then we will show convergence of finite-dimensional distributions $(\langle \Phi_{\eps}, f_i\rangle)_{i\in [m]}$ and identify the limit. \\

\noindent
\textbf{Tightness}
\begin{prop}\label{thm:tightness}
    Let $U\subset \R^d$, $d\geq 2$. Under the scaling $\eps^{-d/2}$, the family $(\Phi_\eps)_{\eps>0}$ is tight in $\mathcal B_{p,q}^{\alpha,\mathrm{loc}}(U)$ for any $\alpha < -d/2$ and $p,q \in [1,\infty]$. The family is also tight in $\mathcal C^\alpha_\mathrm{loc}(U)$ for every $p,q\in[1,\infty]$ and $\alpha < -d/2$.
\end{prop}

Recall that the local Besov space $\mathcal B_{p,q}^{\alpha,\mathrm{loc}}(U)$  was defined in Definition \ref{def:locBes} and the local H\"older space $\mathcal C^\alpha_\mathrm{loc}(U)$ in Definition \ref{def:locHoel}.\\

\noindent
\textbf{Finite-dimensional distributions}

\begin{prop}\label{prop:convWN}
     Let $U\subset \R^d$ and $d\geq 2$. There exists a normalization constant $\chi>0$ such that, for any set of test functions $\left\{f_i\in \mathcal C_c^\infty(U):\, i\in[m],\,m\in\N\right\}$, the random elements $\langle\Phi_\eps,f_i\rangle$ converge in the following sense:
    \[
        \left(\frac{\eps^{-d/2}}{\sqrt \chi}\langle\Phi_\eps,f_i\rangle\right)_{i\in[m]} \overset{d}\longrightarrow \left(\langle W, f_i \rangle \right)_{i\in [m]}
    \]
    as $\eps \to 0$.
\end{prop}



\subsubsection{Proof of Proposition \ref{thm:tightness}}

We will use the tightness criterion given in Theorem 2.30 in \citet{mf}. First we need to introduce some notation. 
Let $f$ and $(g^{(i)})_{1\leq i<2^d}$ be compactly supported test functions of class $\mathcal C^r_c(\R^d)$, $r\in \mathbb{N}$. Let $\Lambda_n \coloneqq \Z^d/2^n$, and let $R>0$ be such that
\begin{equation}\label{eq:support}
    \supp{f} \subset B_0(R) \ , \quad \supp{g^{(i)}} \subset B_0(R) \ , \quad i < 2^d \ .
\end{equation}
Let $K \subset U$ be compact and $k \in \N$. We say that the pair $(K, k)$ is \emph{adapted} if
\[
    2^{-k}R < \dist{(K,U^c)} \ .
\]
We say that the set $\mathcal K$ is a \emph{spanning sequence} if it can be written as
\[
    \mathcal K = \left\{(K_n,k_n): n \in \N\right\} \ ,
\]
where $(K_n)$ is an increasing sequence of compact subsets of $U$ such that $\bigcup_n K_n = U$, and for every $n$ the pair $(K_n, k_n)$ is adapted.


\begin{theorem}[Tightness criterion,{~\citet[Theorem~2.30]{mf}}]\label{thm:criterion}
Let $f, (g^{(i)})_{1\leq i<2^d}$ in $\mathcal C^r_c(\R^d)$ with the support properties mentioned above, and fix $p\in[1,\infty), q\in[1,\infty]$ and $\alpha,\,\beta\in\R$ satisfying $\abs{\alpha},\, \abs{\beta} < r, \alpha<\beta$. Let $(\Phi_m)_{m\in\N}$ be a family of random linear forms on $\mathcal{C}_c^r(U)$, and let $\mathcal K$ be a spanning sequence. Assume that for every $(K, k) \in \mathcal K$ , there exists a constant $c = c(K,k) < \infty$ such that for every $m \in \N$,
\begin{equation}\label{eq:crit_1}
    \sup_{x\in\Lambda_k\cap K}{\E\left[\abs{\big\langle \Phi_m,f\big(2^k(\cdot-x)\big)\big\rangle}^p\right]^{1/p}} \leq c
\end{equation}
and
\begin{equation}\label{eq:crit_2}
    \sup_{x\in\Lambda_n\cap K}{2^{dn}\E\left[\abs{\big\langle \Phi_m,g^{(i)}\big(2^n(\cdot-x)\big)\big\rangle}^p\right]^{1/p}} \leq c \, 2^{-n\beta} \ , \quad i<2^d \ , \ n\geq k \ .
\end{equation}
Then the family $(\Phi_m)_m$ is tight in $\mathcal{B}^{\alpha,\mathrm{loc}}_{p,q}(U)$. If moreover $\alpha < \beta -  d /p$, then the family is also tight in $\mathcal C^\alpha_\mathrm{loc}(U)$.
\end{theorem}

\begin{proof}[Proof of Proposition \ref{thm:tightness}]
We will consider an arbitrary scaling $\eps^{\gamma}, \gamma \in\R$, and then choose an optimal one to make the fields tight. We define $\widetilde\Phi_\eps$ as the scaled version of $\Phi_\eps$, that is,
\[
    \widetilde\Phi_\eps(x) \coloneqq \eps^\gamma \Phi_\eps(x) = \eps^\gamma \sum_{i=1}^d{:\!\left(\nabla_i\Gamma(x)\right)^2\!:} \ , \quad x \in U_\eps \ .
\]
The family of random linear forms $(\Phi_m)_{m\in\N}$ in Theorem~\ref{thm:criterion} is to be identified with the fields $(\widetilde\Phi_\eps)_{\eps>0}$ taking for example $\eps$ decreasing to zero along a dyadic sequence. Now let us expand the expressions \eqref{eq:crit_1} and \eqref{eq:crit_2} in Theorem \ref{thm:criterion}. To simplify notation, let us define $f_{k,x}(\cdot) \coloneqq f\big(2^k(\cdot-x)\big)$ for $k\in\N$ and $x\in \R^d$, and analogously for $g^{(i)}$.

In the proof we will set $p\in 2\N$. This will not affect the generality of our results because of the embedding of local Besov spaces described in Lemma~\ref{lemma:embedding}.
This means that we can read \eqref{eq:crit_1} forgetting the absolute value in the left-hand side. Let us rewrite the $p$-th moment of $\big\langle\widetilde\Phi_\eps,f_{k,x}\big\rangle$ as
\begin{equation}\label{eq:crit_1_1}
   0\le \E\left[{\big\langle \widetilde\Phi_\eps,f_{k,x}\big\rangle}^p\right] = \eps^{\gamma p}\, \E\left[\int_{U^p}\Phi_\eps\left(\floor{x_1/\eps}\right)\cdots\Phi_\eps\left(\floor{x_p/\eps}\right) f_{k,x}(x_1)\cdots f_{k,x}(x_p)\, \d x_1\cdots\d x_p \right]\ .
\end{equation}
We will seek for a more convenient expression to work with. If we allow ourselves to slightly abuse the notation for $\widetilde\Phi_\eps$, then we can express it in a piece-wise continuous fashion as
\[
    \widetilde\Phi_\eps(x) = \eps^{\gamma} \sum_{y\in U_\eps} \1_{S_1(y)}(x) \sum_{i=1}^d{:\!\left(\nabla_i\Gamma(y)\right)^2\!:} = \eps^{\gamma} \sum_{y\in U_\eps} \1_{S_1(y)}(x) \Phi_\eps(y) \ ,
\]
where $S_a(y)$ is the square of side-length $a$ centered at $y$. Under a change of variables, if we define $U^\eps \coloneqq U\cap\eps\Z^2$ (mind the superscript and the definition which is different from that of $U_\eps$ in Section \ref{sec:not}) then
\[
    \widetilde\Phi_\eps(x) = \eps^{\gamma} \sum_{y\in U^\eps} \1_{S_\eps(y/\eps)}(x) \Phi_\eps(y/\eps) \ .
\]
This way, expression \eqref{eq:crit_1_1} now reads
\[
    \E\left[{\big\langle \widetilde\Phi_\eps,f_{k,x}\big\rangle}^p\right] = \eps^{\gamma p}\, \E\left[\sum_{y_1,\dots,y_p\in U^\eps} {\Phi_\eps(y_1/\eps)\cdots\Phi_\eps(y_p/\eps)}\prod_{j=1}^p{\int_{S_\eps(y_j)}{f_{k,x}(z) \,\d z}} \right]\ ,
\]
Therefore the left-hand side of expression \eqref{eq:crit_1} from Theorem \ref{thm:criterion} is upper-bounded by
\begin{equation}\label{eq:first}
    \eps^{\gamma} \sup_{x\in\Lambda_k \cap K}{\left[\sum_{y_1,\dots,y_p\in U^\eps} \E\left[\Phi_\eps(y_1/\eps)\cdots\Phi_\eps(y_p/\eps)\right]\prod_{j=1}^p{\int_{S_\eps(y_j)}f_{k,x}(z) \,\d z}\right]^{1/p}} \ .
\end{equation}
Analogously, expression \eqref{eq:crit_2} from Theorem \ref{thm:criterion} reads
\begin{equation}\label{eq:second}
    \eps^{\gamma} \, 2^{dn}\sup_{x\in\Lambda_n \cap K}{\left[\sum_{y_1,\dots,y_p\in U^\eps} {\E\left[\Phi_\eps(y_1/\eps)\cdots\Phi_\eps(y_p/\eps)\right]}\prod_{j=1}^p{\int_{S_\eps(y_j)}{g_{n,x}^{(i)}(z)} \,\d z}\right]^{1/p}} \ .
\end{equation}

Choose $\mathcal K = (K_n,n)_{n\in\N}$ with
\[
    K_n = \big\{x\in\R^d \mid \dist{(x,U^c)}\geq(2+\delta)R2^{-n}\big\} \ ,
\]
for some $\delta > 0$ and $R$ such that \eqref{eq:support} holds.

Let us first consider \eqref{eq:second}. Given that $\supp{g^{(i)}\big(2^n(\cdot-x)\big)} \subset B_x(R2^{-n})$ we can restrict the sum over $y_j$ to the set
\[
    \Omega_{n,x} = \left\{y\in U^\eps \mid \d(y,x)<2^{-n}R+\eps\sqrt{d}/2\right\} \ .
\]
We now bound \eqref{eq:second} separately for the cases $2^n \geq R\eps^{-1}$ and $2^n < R\eps^{-1}$.

If $2^n \geq R\eps^{-1}$, we have
\begin{multline*}
    \sum_{y_1,\dots,y_p\in U^\eps} {\E\left[\Phi_\eps(y_1/\eps)\cdots\Phi_\eps(y_p/\eps)\right]}\prod_{j=1}^p{\int_{S_\eps(y_j)}g_{n,x}^{(i)}(z) \,\d z} \leq \\
    \leq \sum_{y_1,\dots,y_p\in \Omega_{n,x}} {\E\left[\Phi_\eps(y_1/\eps)\cdots\Phi_\eps(y_p/\eps)\right]}\prod_{j=1}^p{\int_{S_\eps(y_j)}g_{n,x}^{(i)}(z) \,\d z} \ .
\end{multline*}
The sum over $\Omega_{n,x}$ can be bounded by a sum over a finite amount of points independent of $n$, since under the condition $2^n \geq R\eps^{-1}$ the set $\Omega_{x,n}$ has at most $3^d$ points for any $x$ and $n$. Using the fact that
\[
    \int_{S_\eps(y_j)} \abs{g_{n,x}^{(i)}(z)} \,\d z \leq 2^{-dn}
\]
we obtain
\[
    \sum_{y_1,\dots,y_p\in \Omega_{n,x}} {\E\left[\left|\Phi_\eps(y_1/\eps)\cdots\Phi_\eps(y_p/\eps)\right|\right]}\prod_{j=1}^p{\int_{S_\eps(y_j)}{g_{n,x}^{(i)}(z) \,\d z}} \lesssim 2^{-dpn} \ ,
\]
which gives the bound
\[
    \eps^{\gamma} \, 2^{dn}\sup_{x\in\Lambda_n \cap K}{\left[\sum_{y_1,\dots,y_p\in U^\eps} {\E\left[\Phi_\eps(y_1/\eps)\cdots\Phi_\eps(y_p/\eps)\right]}\prod_{j=1}^p{\int_{S_\eps(y_j)}{g_{n,x}^{(i)}(z) \,\d z}}\right]^{1/p}} \lesssim \eps^{\gamma} \ .
\]
Then, for any $\gamma\leq0$ we can bound the above expression by a constant multiple of $ 2^{-\gamma n}$. 
On the other hand, if $2^n < R\eps^{-1}$, we have
\[
    \int_{S_\eps(y_j)}\abs{g_{n,x}^{(i)}(z)}\d z \leq \eps^d \ .
\]
We also note that
\[
    \Omega_{n,x} \subset S_{\eps,x} \coloneqq \left[x - 2R2^{-n},x + 2R2^{-n}\right]^d \cap \eps\Z^d \ .
\]
Using this and calling $N\coloneqq\lfloor2R2^{-n}\eps^{-1}\rfloor$, we obtain
\[
    \sum_{y_1,\dots,y_p\in \Omega_{n,x}} {\E\left[\Phi_\eps(y_1/\eps)\cdots\Phi_\eps(y_p/\eps)\right]} \leq \sum_{y_1,\dots,y_p\in \llbracket-N,N\rrbracket^d} {\E\left[\Phi_\eps(y_1)\cdots\Phi_\eps(y_p)\right]} \ .
\]
Let us first study the behaviour of this expression for $p=2$. By Corollary \ref{cor:covariance_bound} we get
\begin{multline*}
    \sum_{y_1,y_2\in \llbracket-N,N\rrbracket^d} {\E\left[\Phi_\eps(y_1)\Phi_\eps(y_2)\right]} \lesssim_K \sum_{\substack{y_1,y_2\in \llbracket-N,N\rrbracket^d\\\mathstrut y_1 = y_2}} 1 \,+ \sum_{\substack{y_1,y_2\in \llbracket-N,N\rrbracket^d\\\mathstrut y_1 \neq y_2}} \frac{1}{\left|y_1-y_2\right|^{2d}} \\ \lesssim N^d + \sum_{y_1 \in \llbracket-N,N\rrbracket^d} \int_1^{2\sqrt2N}\frac{r^{d-1}}{r^{2d}}\d r
    = N^d + \sum_{y_1 \in \llbracket-N,N\rrbracket^d} \frac1d \left(1 - 2^{-3d/2} N^{-d}\right) \lesssim N^d \ .
\end{multline*}
Observe that Theorem \ref{thm:criterion} allows the constant $c$ to depend on $k$ and $K$ so the symbol $\lesssim_K$ is not an issue. Let us now analyze $\E\left[\Phi_\eps(y_1)\dots\Phi_\eps(y_p)\right]$ for an arbitrary $p$. Looking at expression \eqref{eq:cumulants2} we observe the following: any given partition $\pi\in\Pi([p])$ with no singletons can be expressed as $\pi = \{B_1,\dots,B_k\}$, with $1\leq k\leq p$ such that $\sum_{1\leq i\leq k} n_i = p$, with $n_i \coloneqq \abs{B_i}$. Then the cumulant corresponding to any given $B_i$ (see Corollary \ref{cor:cumulants}) is proportional to a sum (over $\sigma \in S_\mathrm{cycl}(B_i)$ and $\eta:B_i\to\mathcal E$) of terms of the form
\[
    \prod_{j\in B_i} \nabla_{\eta(j)}^{(1)} \nabla_{\eta(\sigma(j))}^{(2)} G_{U_\eps}\big(y_j, y_{\sigma(j)}\big) \ .
\]
Using \eqref{eq:two_durre} we can bound this expression (up to a constant) by
\[
    \prod_{j\in B_i} \min{\left\{\big|y_{j} - y_{\sigma(j)}\big|^{-d},\,1\right\}} \ ,
\]
where the minimum takes care of the case in which $B_i$ has repeated values. Lemma \ref{lemma:sum_p_point_function} implies that $\E\left[\Phi_\eps(y_1)\dots\Phi_\eps(y_p)\right]$ can be bounded (up to a constant depending on $K$) by a sum of terms of magnitude
\[
    \prod_{i=1}^{\abs{\pi}} N^{\frac{n_i}{2}+d-1} = N^{(d-1)|\pi|+\frac{p}{2}} \ .
\]
Since the sum takes place over partitions of the set $[p]$ with no singletons, putting everything back into~\eqref{eq:cumulants2} we see that the term with the largest value of $\abs{\pi}$ will dominate for large $N$. For $p$ even this happens when $\pi$ is composed of cycles of two elements, in which case $\abs{\pi} = p/2$. Hence,
\[
    \sum_{y_1,\dots,y_p \in \llbracket-N,N\rrbracket^d} \E\big[\Phi_\eps(y_1)\cdots\Phi_\eps(y_p)\big] \lesssim_K N^\frac{dp}{2}
\]
for $p$ even. Finally,\
\[
    \eps^{\gamma} \, 2^{dn}\sup_{x\in\Lambda_n \cap K}{\left[\sum_{y_1,\dots,y_p\in U^\eps} {\E\left[\Phi_\eps(y_1/\eps)\cdots\Phi_\eps(y_p/\eps)\right]}\prod_{j=1}^p{\int_{S_\eps(y_j)}{g_{n,x}^{(i)}(z) \,\d z}}\right]^{1/p}} \lesssim_K 2^\frac{dn}{2} \eps^{\gamma+\frac{d}{2}} \ .
\]
If $\gamma \geq -d/2$ then we can bound the above expression by a constant multiple of $ 2^{\frac{dn}{2}} 2^{-\left(\gamma+\frac{d}{2}\right)n} = 2^{-\gamma n}$. Otherwise, we cannot bound it uniformly in $\eps$, as the bound depends increasingly on $\eps$ as it approaches 0.

Now we need to obtain similar bounds for \eqref{eq:crit_1}, which applied to our case takes the expression given in \eqref{eq:first}. For the case $2^k \geq R\eps^{-1}$ we have
\[
    \eps^{\gamma} \sup_{x\in\Lambda_k \cap K}{\left[\sum_{y_1,\dots,y_p\in U^\eps} {\E\left[\Phi_\eps(y_1/\eps)\cdots\Phi_\eps(y_p/\eps)\right]}\prod_{j=1}^p{\int_{S_\eps(y_j)}{f_{k,x}(z) \,\d z}}\right]^{1/p}} \lesssim \eps^\gamma \,2^{-dk} < \eps^{\gamma+d} \ ,
\]
which is bounded by some $c = c(K,k)$ whenever $\gamma \geq -d$. If $2^k < R\eps^{-1}$ instead we get
\[
    \eps^{\gamma} \sup_{x\in\Lambda_k \cap K}{\left[\sum_{y_1,\dots,y_p\in U^\eps} {\E\left[\Phi_\eps(y_1/\eps)\cdots\Phi_\eps(y_p/\eps)\right]}\prod_{j=1}^p{\int_{S_\eps(y_j)}{f_{k,x}(z) \,\d z}}\right]^{1/p}} \lesssim_K \eps^{\gamma+\frac{d}{2}} \,2^{-\frac{dk}{2}} \ .
\]
As before, only if $\gamma \geq -{d}/{2}$ we have the required bound.

Theorem \ref{thm:criterion} now implies that under scaling $\eps^{-d/2}$ the family $(\Phi_\eps)_{\eps>0}$ is tight in $\mathcal B_{p,q}^{\alpha,\mathrm{loc}}(U)$ for any $\alpha < -{d}/{2}$, any $q\in[1,\infty]$ and any $p \geq 2$ and even. Using Lemma \ref{lemma:embedding} this holds for any $p \in [1,\infty]$. This way, the family is also tight in $\mathcal C^\alpha_\mathrm{loc}(U)$ for every $\alpha < -{d}/{2}$.
\end{proof}

\begin{remark}
    Observe that the scaling $\eps^{-d}$ (the one used for the joint moments in Theorem \ref{thm:cumulants}) is outside the range of $\gamma$ required for the tightness bounds, and therefore it will give a trivial scaling.
\end{remark}



==> wn.tex <==
\subsubsection{Proof of Proposition \ref{prop:convWN}}

The proof of this proposition will be divided into three parts. Firstly, we will determine the normalizing constant $\chi$ and show that it is well-defined, in the sense that it is a strictly positive finite constant. Secondly, recalling Definition~\ref{def:cum_single}, we will demonstrate that the $n$-th cumulant $\kappa_n(\langle \Phi_{\eps}, f\rangle)$ of each random variable $\langle \Phi_{\eps}, f\rangle$, $f\in L^2(U)$, vanishes for $n\geq 3$ and finally that the second cumulant $\kappa_2(\langle \Phi_{\eps}, f\rangle)$, which is equal to the covariance, converges to the appropriate one corresponding to that of white noise. The ideas are partially inspired from \citet[Section 3.6]{durrethesis}.

For the rest of this Subsection we will work with test functions $f\in C_c^\infty(U)$. The lifting of the results to every $f\in L^2(U)$ follows by a standard density argument~\cite[Chapter 1, Section 3]{janson}. Let us first derive a convenient representation of the action $\langle \Phi_{\eps}, f\rangle$ defined in Equation \eqref{def:action}. More precisely, defining $\langle \Phi_{\eps}, f\rangle_S$ as
\[
    \langle \Phi_{\eps}, f\rangle_S \coloneqq \sum_{v\in U_\eps} {f(\eps v)\Phi_\eps(v)} \ ,
\]
for any test function $f\in \mathcal C^{\infty}_c(U)$ we can write
\[
\begin{split}
\langle \Phi_{\eps}, f\rangle & = \eps^d \langle \Phi_{\eps}, f\rangle_S + R_{\eps}(f) \ ,
\end{split}
\]
where $R_{\eps}(f)$ denotes the reminder term that goes to $0$ in $L^2$, as we show in the next lemma.

\begin{lemma}
    Let $U\subset \R^d$, $d\geq 2$. For any test function $f\in\mathcal C^\infty_c(U)$ as $\eps\to0$ it holds that
    \begin{equation}\label{eq:difference_actions}
        \abs{R_{\eps}(f)} \xrightarrow{L^2} 0 \ .
    \end{equation}
\end{lemma}

\begin{proof}
Observe that
\[
    \langle\Phi_\eps,f\rangle = \int_U \Phi_\eps\left(\floor{x/\eps}\right)f(x) \d x = \sum_{x \in U_\eps}\Phi_\eps(x) \int_{A_x} f(y) \d y \ ,
\]
where $A_x \coloneqq \left\{a\in U : \floor{a/\eps}=x\right\}$. It is easy to see that $\abs{A_x} \leq \eps^d$, and given that the support of $f$ is compact and strictly contained in $U$, for $\eps$ sufficiently small (depending on $f$), the distance between this support and the boundary $\partial U$ will be larger than $\sqrt{d}\eps$. So there is no loss of generality if we assume that~$\abs{A_x} = \eps^d$.

Now, we can rewrite \eqref{eq:difference_actions} as
\begin{equation}\label{eq:I_factor}
    \abs{\sum_{x\in U_\eps}\Phi_\eps(x) \left(\int_{A_x} f(y) \d y - \eps^d \, f(\eps x)\right)} = \abs{\sum_{x\in U_\eps}\eps^d \, \Phi_\eps(x) \left(\frac{1}{|A_x|}\int_{A_x} f(y) \d y - \, f(\eps x)\right)} \ .
\end{equation}
Let us call $\mathcal I(x)$ the term
\[
\mathcal I(x) \coloneqq \frac{1}{|A_x|}\int_{A_x} f(y) \d y - \, f(\eps x) \ .
\]
The set $A_x$ is not a Euclidean ball, but it has bounded eccentricity (see \citet[Corollary 1.7]{stein2009real}). Therefore we can apply the Lebesgue differentiation theorem to claim that $\mathcal I(x)$ will be of order $o(1)$, where the rate of convergence possibly depends on $x$ and $f$.

To see statement \eqref{eq:difference_actions}, we square the expression in~\eqref{eq:I_factor} and take its expectation, obtaining
\begin{equation}\label{eq:help_eq}
    \E\left[\bigg|\sum_{x\in U_\eps}\eps^d \, \Phi_\eps(x) \,\mathcal I(x)\bigg|^2\right] \leq \eps^{2d}\, \E\left[\sum_{x\in U_\eps}\Phi_\eps^2(x)\right]\left(\sum_{x\in U_\eps}\mathcal I^2(x)\right)
\end{equation}
where we used the Cauchy-Schwarz inequality. By Corollary \ref{cor:covariance_bound} the expectation on the right-hand side can be bounded as
\[
    \E\left[\sum_{x\in U_\eps}\Phi_\eps^2(x)\right] \lesssim \sum_{x\in U_\eps} 1 = \mathcal O\big(\eps^{-d}\big)
\]
while the second term in~\eqref{eq:help_eq} is of order $o(\eps^{-d})$. With the outer factor $\eps^{2d}$~\eqref{eq:help_eq} goes to $0$, as we wanted to show.
\end{proof}

Let us remark that, by the previous lemma, proving finite-dimensional convergence of $\left\{\frac{\eps^{-d/2}}{\sqrt{\chi}}\langle \Phi_\eps,f_p\rangle:\,p\in[m]\right\}$ will be equivalent to proving finite-dimensional convergence of $\left\{\frac{\eps^{d/2}}{\sqrt{\chi}}\langle \Phi_\eps,f_p\rangle_S:\,p\in[m]\right\}$.



\subsubsection*{Definition of $\chi$}

\begin{lemma}\label{lemma:chi}
Let $G_0(\cdot, \cdot)$ be the Green's function on $\mathbb{Z}^d$ defined in Section \ref{sec:GFF}. The constant
    \[
        \chi \coloneqq 2\sum_{v\in\Z^d} \sum_{i,j\in[d]} \left(\nabla_i^{(1)}\nabla_j^{(2)}G_0(0,v)\right)^2
    \]
    is well-defined. In particular $\chi \in (8,\,+\infty)$.
\end{lemma}

\begin{proof}
Let us define $\kappa_0$ as
\begin{equation}\label{eq:kappa_0}
    \kappa_0(v,w) \coloneqq 2\sum_{i,j\in[d]} \left(\nabla_i^{(1)}\nabla_j^{(2)}G_0(v,w)\right)^2 \ .
\end{equation}
By translation invariance we notice that $\kappa_0(v,w) = \kappa_0(0,w-v)$. Moreover, using Lemma~\ref{lemma:lemma_29_durre}, we have that as $|v|\to+\infty$
\[
    \kappa_0(0,\,v)\lesssim |v|^{-2d}
\]
so that we can bound $\chi$ from above by
\[
    \chi = \sum_{v\in\Z^d} \kappa_0(0,v) \lesssim \,1 + \sum_{v\in\Z^d\setminus\{0\}} |v|^{-2d} < +\infty \ .
\]

For the lower bound, since $\kappa_0(0,v) \geq 0 $ for all $ v\in\Z^d$ we can take $v = 0$. Choosing the differentiation directions $i=j=1$ in \eqref{eq:kappa_0} we get the term $2\big(\nabla_1^{(1)}\nabla_1^{(2)}G_0(0,0)\big)^2$, which can be expressed as $8\left(G_0(0,0)-G_0(e_1,0)\right)^2$ using translation and rotation invariance of $G_0$. Now, by definition
\[
    \Delta G_0(0,0) = \frac{1}{2d} \sum_{x\in\Z^d:|x|=1}\left(G_0(x,0)-G_0(0,0)\right) = -1 \ ,
\]
from which $G_0(0,0) - G_0(e_1,0) = 1$. This implies that $\chi \geq 8$, and the lemma follows.
\end{proof}



\subsubsection*{Vanishing cumulants $\kappa_n$ for $n\geq 3$}

\begin{lemma}
For $n\geq3$, $f\in C_c^\infty(U)$, the cumulants $\kappa_n \left(\eps^{d/2}\langle \Phi_\eps,f\rangle_S\right)$ go to $0$ as $\eps\to0$.
\end{lemma}

\begin{proof}
Recall that by Corollary \ref{cor:cumulants}, for $n\geq2$, the $n$-th cumulant satisfies
\begin{equation}\label{eq:nth_cumulant}
    \kappa_n\left(\eps^{d/2}\langle \Phi_\eps,f\rangle_S\right) = \eps^\frac{nd}{2} \sum_{v_1,\ldots,v_n \in D_\eps} \kappa\left(\Phi_\eps(v_i):i\in[n]\right) \prod_{j=1}^n f(\eps v_j) \ ,
\end{equation}
with $D\coloneqq \supp f$, which is compact inside $U$. The goal now is to show that
\[
    \eps^\frac{nd}{2} \sum_{v_1,\ldots,v_n \in D_\eps} \abs{\kappa\left(\Phi_\eps(v_i):i\in [n]\right)} \ \longrightarrow 0
\]
as $\eps\to 0$.

First, we note from the cumulants expression \eqref{eq:cumulants3} and bound \eqref{eq:two_durre} in Lemma \ref{lemma:bound_2_points_durre} that, for any set $V$ of (possibly repeated) points of $D_\eps$, with $\abs{V} = n$, we have
\[
    \abs{\kappa\left(\Phi_\eps(v):v \in V\right)} \lesssim_{D,n} \sum_{\sigma\in S^0_\mathrm{cycl}(V)}\prod_{v\in V} \min{\left\{\left|v-\sigma(v)\right|^{-d},\,1\right\}} \ .
\]
Using the above expression and Lemma \ref{lemma:sum_p_point_function}, it is immediate to see that, if $V$ has $m$ distinct points with $1\leq m\leq n$,
\[
    \sum_{\substack{v_1,\ldots,v_n \in D_\eps\\\mathstrut\text{$m$ distinct points}}} \abs{\kappa\left(\Phi_\eps(v_i):i\in [n]\right)} = \mathcal{O}_D\left(\eps^{-\frac{m}{2}-d+1}\right) \lesssim \mathcal{O}_D\left(\eps^{-\frac{n}{2}-d+1}\right)
\]
so that
\[
    \eps^\frac{nd}{2} \sum_{v_1,\ldots,v_n \in D_\eps} \abs{\kappa\left(\Phi_\eps(v_i):i\in [n]\right)} = \mathcal{O}_D\left(\eps^{\frac{1}{2}(d-1)(n-2)}\right) \ .
\]
We observe in particular that for $d\geq2$ this expression goes to $0$ for any $n\geq3$. Furthermore, going back to \eqref{eq:nth_cumulant}, since $f$ is uniformly bounded this shows that for $n\geq3$ the cumulants $\kappa_n$ go to $0$ as $\eps\to0$, as we wanted to show.
\end{proof}


\subsubsection*{Covariance structure $\kappa_2$}

\begin{lemma}
For any two functions $f_p,f_q \in \mathcal C^{\infty}_c(U)$, with $p,q\in[m]$ for $m \in\N$, we have
\[
    \eps^d\, \kappa\left(\langle\Phi_\eps,f_p\rangle_S,\langle\Phi_\eps,f_q\rangle_S\right) \xrightarrow{\eps\to0} \chi \int_U f_p(x) f_q(x) \d x \ .
\]
\end{lemma}

\begin{proof}
Without loss of generality we define the compact set $D\subset U$ as the intersection of the supports of $f_p$ and $f_q$. Then
\begin{equation}\label{eq:k_n2}
    \eps^d \,\kappa\left(\langle\Phi_\eps,f_p\rangle_S,\langle\Phi_\eps,f_q\rangle_S\right) = \eps^d \sum_{v,w \in D_\eps} f_p(\eps v) f_q(\eps w) \,\kappa\left(\Phi_\eps(v),\Phi_\eps(w)\right) \ .
\end{equation}
From Theorem \ref{thm:cumulants}, we know the exact expression of $\kappa\left(\Phi_\eps(v),\Phi_\eps(w)\right)$, given by
\begin{equation}\label{eq:2point}
    \kappa\left(\Phi_\eps(v),\Phi_\eps(w)\right) = 2\sum_{i,j\in[d]} \left(\nabla_i^{(1)}\nabla_j^{(2)}G_{U_\eps}(v,w)\right)^2 \ .
\end{equation}
Recall the constant $\kappa_0(v,w)$, defined in \eqref{eq:kappa_0}. We will approximate $\kappa\left(\Phi_\eps(v),\Phi_\eps(w)\right)$ by $\kappa_0(v,w)$ and then plug it in \eqref{eq:k_n2}. In other words, we will approximate $G_{U_\eps}(\cdot,\cdot)$ by $G_0(\cdot,\cdot)$. First we split Equation \eqref{eq:k_n2} into two parts:

\begin{multline}\label{eq:split_sum}
    \eps^d \,\kappa\left(\langle\Phi_\eps,f_p\rangle_S,\langle\Phi_\eps, f_q\rangle_S\right) = \eps^d \sum_{\substack{v,w \in D_\eps\\|v-w|\leq1/\sqrt{\eps}}} f_p(\eps v) f_q(\eps w) \,\kappa\left(\Phi_\eps(v),\Phi_\eps(w)\right) \\
    + \eps^d \sum_{\substack{v,w \in D_\eps\\|v-w|>1/\sqrt{\eps}}} f_p(\eps v) f_q(\eps w)\, \kappa\left(\Phi_\eps(v),\Phi_\eps(w)\right) \ .
\end{multline}
The second term above can be easily disregarded: remember that the cumulant for two random variables equals their covariance, so using Corollary \ref{cor:covariance_bound} we get
\[
    \eps^d \sum_{\substack{v,w \in D_\eps\\\abs{v-w}>1/\sqrt{\eps}}} f_p(\eps v) f_q(\eps w) \,\kappa\left(\Phi_\eps(v),\Phi_\eps(w)\right) \lesssim \eps^d \sum_{\substack{v,w \in D_\eps\\|v-w|>1/\sqrt{\eps}}} |v-w|^{-2d} \lesssim \sum_{\substack{z \in \Z^d\\|z|>1/\sqrt{\eps}}} |z|^{-2d} \ ,
\]
which goes to $0$ as $\eps\to0$. For the first sum in~\eqref{eq:split_sum}, let us compute the error we are committing when replacing $G_{U_\eps}$ by $G_0$. We notice that
\[
    \max_{i,j\in[d]} \sup_{v,w\in D_\eps} \sup_{\eps\in(0,\eps_D]}  \abs{\nabla_i^{(1)}\nabla_j^{(2)} G_{U_\eps}(v,w)} \leq  c_D
\]
justified by~\eqref{eq:two_durre} in Lemma \ref{lemma:bound_2_points_durre}, combined with
\[
    \max_{i,j\in[d]} \sup_{v,w\in \Z^d} \abs{\nabla_i^{(1)}\nabla_j^{(2)} G_{0}(v,w)}\le c
\]
for some $c>0$, which is a consequence of Lemma~\ref{lemma:lemma_29_durre}. Recalling that $|a^2-b^2|= |a-b||a+b|$ for any real numbers $a,\,b$, and setting
\[
    a\coloneqq \nabla_i^{(1)}\nabla_j^{(2)} G_{U_\eps}(v,w)
\]
and 
\[
    b\coloneqq\nabla_i^{(1)}\nabla_j^{(2)} G_0(v,w) \ ,
\]
together with \eqref{eq:one_durre} from Lemma \ref{lemma:bound_2_points_durre}, we obtain

\begin{equation*}\label{eq:approx_sum_G}
   \sum_{i,j\in[d]} \left(\nabla_i^{(1)}\nabla_j^{(2)}G_{U_\eps}(v,w)\right)^2= \sum_{i,j\in[d]} \left(\nabla_i^{(1)}\nabla_j^{(2)}G_0(v,w)\right)^2 + \mathcal{O}\big(\eps^d\big) \ .
\end{equation*}

We can use this approximation in the first summand in \eqref{eq:split_sum} and obtain
\begin{equation}\label{eq:approx}
    \eps^d \sum_{\substack{v,w \in D_\eps\\|v-w|\leq1/\sqrt{\eps}}} f_p(\eps v) f_q(\eps w)\, \kappa\left(\Phi_\eps(v),\Phi_\eps(w)\right) = \eps^d \sum_{\substack{v,w \in D_\eps\\|v-w|\leq1/\sqrt{\eps}}} f_p(\eps v) f_q(\eps w) \,\kappa_0(v,w) + \mathcal O\big(\eps^{d/2}\big) \ ,
\end{equation}
since $\abs{\left\{v,w \in D_\eps:|v-w| < 1/\sqrt{\eps}\right\}} = \mathcal O\big(\eps^{-\frac{3}{2}d}\big)$. Now, given that both $f_p$ and $f_q$ are in $\mathcal C_c^\infty(U)$, they are also Lipschitz continuous. Hence 
\[
    \eps^d \sum_{\substack{v,w \in D_\eps\\|v-w|\leq1/\sqrt{\eps}}}\abs{f_q(\eps v)-f_q(\eps w)} \abs{\kappa_0(v,w)} \lesssim \eps^d \sum_{\substack{v,w \in D_\eps\\1\leq |v-w|\leq1/\sqrt{\eps}}}\frac{\sqrt{\eps}}{|v-w|^{2d}} = o(1) \ ,
\]
so that we can replace, up to a negligible error, $f_q(\eps w)$ by $f_q(\eps v)$ in \eqref{eq:approx}, getting
\[
    \eps^d\, \kappa\left(\langle\Phi_\eps,f_p\rangle_S,\langle\Phi_\eps,f_q\rangle_S\right) = \eps^d \sum_{\substack{v,w \in D_\eps\\|v-w|\leq1/\sqrt{\eps}}} f_p(\eps v) f_q(\eps v)\, \kappa_0(v,w) +  o(1) \ .
\]
Finally the translation invariance of $\kappa_0$ implies
\[
    \lim_{\eps\to0} \,\eps^d\, \kappa\left(\langle\Phi_\eps,f_p\rangle_S,\langle\Phi_\eps,f_q\rangle_S\right) = \sum_{v\in\Z^d} \kappa_0(0,v) \int_U f_p(x) f_q(x) \d x
\]
as claimed.
\end{proof}

